Private Online Prediction from Experts: Separations and Faster Rates

Online prediction from experts is a fundamental problem in machine learning and several works have studied this problem under privacy constraints. We propose and analyze new algorithms for this problem that improve over the regret bounds of the best existing algorithms for non-adaptive adversaries. For approximate differential privacy, our algorithms achieve regret bounds of $\tilde{O}(\sqrt{T \log d} + \log d/\varepsilon)$ for the stochastic setting and $\tilde{O}(\sqrt{T \log d} + T^{1/3} \log d/\varepsilon)$ for oblivious adversaries (where $d$ is the number of experts). For pure DP, our algorithms are the first to obtain sub-linear regret for oblivious adversaries in the high-dimensional regime $d \ge T$. Moreover, we prove new lower bounds for adaptive adversaries. Our results imply that unlike the non-private setting, there is a strong separation between the optimal regret for adaptive and non-adaptive adversaries for this problem. Our lower bounds also show a separation between pure and approximate differential privacy for adaptive adversaries where the latter is necessary to achieve the non-private $O(\sqrt{T})$ regret.

==> conclusion.tex <==


\section{Conclusion}
In this work, we studied differentially private online learning problems in the realizable setting, and developed algorithms with improved rates compared to the non-realizable setting. However, several questions remain open in this domain. First, our near-optimal algorithms for DP-OPE obtain $\log^{1.5}(d)/\diffp$ regret, whereas the lower bound we have is $\Omega(\log(d)/\diffp)$. Hence, perhaps there are better algorithms with tighter logarithmic factors than our sparse-vector based algorithms. Additionally, for DP-OCO, our algorithms are optimal only for low-dimensional setting, and there remains polynomial gaps in the high-dimensional setting. Finally, optimal rates for both problems (DP-OPE and DP-OCO) are still unknown in the general non-realizable setting.


==> realizable-LB.tex <==
\section{Lower bounds}
\label{sec:real-LB}
In this section, we prove lower bounds for private experts in the realizable setting which show that our upper bounds are nearly-optimal up to logarithmic factors. The lower bound demonstrates that a logarithmic dependence on $d$ is necessary even in the realizable setting. Note that for DP-OCO in the realizable setting, a lower bound of $d/\diffp$ for pure DP follows from known lower bounds for DP-SCO in the interpolation regime~\cite{AsiChChDu22} using online-to-batch conversions~\cite{Hazan16}.

The following theorem states our lower bound for DP-OPE.
\begin{theorem}
\label{thm:lb-obl-experts}
    Let $\diffp \le 1/10$ and $\delta \le \diffp/d$.
    If $\A$ is $(\diffp,\delta)$-DP then there is an oblivious adversary such that $\min_{x\in[d]} \sum_{t=1}^T \ell_t(x) = 0$ and 
    \begin{equation*}
        \E\left[\sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x)\right]
        \ge \Omega \left( \frac{\log(d)}{\diffp} \right).
    \end{equation*}
\end{theorem}
\begin{proof}
    Let $\ell^0(x)=0$ for all $x$ and for $j \in [d]$
    let $\ell^j(x)$ be the function that has $\ell^j(x)=0$ for $x=j$ and otherwise $\ell^j(x)=1$. The oblivious adversary picks one of the following $d$ sequences uniformly at random: $\Ds^j = (\underbrace{\ell^0,\dots,\ell^0}_{T-k},\underbrace{\ell^j,\dots,\ell^j}_{k})$ where $k = \frac{\log d}{2 \diffp}$ and $j \in [d]$. Assume towards a contradiction that the algorithm obtains regret $\log(d)/(32\diffp)$. This implies that there exists $d/2$ sequences such that the algorithm obtains expected regret $\log(d)/(16\diffp)$ where the expectation is only over the randomness of the algorithm. Assume without loss of generality these sequences are $\Ds^1,\dots,\Ds^{d/2}$. Let $B_j$ be the set of outputs that has low regret on $\Ds^j$, that is,
    \begin{equation*}
        B_j = \{ (x_1,\dots,x_T) \in [d]^T: \sum_{t=1}^T \ell^j(x_t) \le \log(d)/(8\diffp) \}.
    \end{equation*}
    Note that $B_j \cap B_{j'} = \emptyset$ since 
    if $x_{1:T} \in B_j$ then at least $3k/4 = 3\log(d)/(8\diffp)$ of the last $k$ outputs must be equal to $j$. Now Markov inequality implies that 
    % \begin{equation*}
    %     \P(\A(\Ds^j) \notin B_j) \le 1/10d.
    % \end{equation*}
    % Moreover, group privacy also gives
    % \begin{align*}
    % \P(\A(\Ds^{j}) \notin B_{j'}) 
    %     & \le e^{k\diffp} \P(\A(\Ds^{j'}) \notin B_{j'}) + k e^{(k-1)\diffp} \delta \\
    %     & \le \sqrt{d}/10d + \log(d) \sqrt{d} \delta/(2\diffp) \\
    %     & \le 1/4.
    % \end{align*}
    % Overall we get that $\P(\A(\Ds^{j}) \in B_{j'}) \ge 3/4 $ for all $j'$. This gives a contradiction as 
    % \begin{align*}
    % \P(\A(\Ds^{j}) \in B_1 \cap B_2 \cap B_3) 
    %     \ge 1/4 >0,
    % \end{align*}
    % which is a contradiction as $B_1 \cap B_2 \cap B_3 = \emptyset$.
    \begin{equation*}
        \P(\A(\Ds^j) \in B_j) \ge 1/2.
    \end{equation*}
    Moreover, group privacy gives
    \begin{align*}
    \P(\A(\Ds^{j}) \in B_{j'}) 
        & \ge e^{-k\diffp} \P(\A(\Ds^{j'}) \in B_{j'}) - k e^{-\diffp} \delta \\
        & \ge \frac{1}{2 \sqrt{d}} - \frac{\log(d)}{2\diffp} \delta \\
        & \ge \frac{1}{4 \sqrt{d}},
    \end{align*}
    where the last inequality follows since $\delta \le \diffp/d$.
    Overall we get that 
    \begin{align*}
        \frac{d/2-1}{4\sqrt{d}}  \le 
        \P(\A(\Ds^{j}) \notin B_{j}) 
         \le \frac{1}{2}  ,
    \end{align*}
    which is a contradiction for $d \ge 32$.
\end{proof}

==> realizable-abstract.tex <==

\begin{abstract}
    We consider online learning problems in the realizable setting, where there is a zero-loss solution, and propose new Differentially Private (DP) algorithms that obtain near-optimal regret bounds.
    For the problem of online prediction from experts, we design new algorithms 
    that obtain near-optimal regret $\wt O \big( \diffp^{-1} \log^{1.5}{d} \big)$ where $d$ is the number of experts. 
    This significantly improves over the best existing regret bounds for the DP non-realizable setting which are $\wt O \big( \diffp^{-1} \min\big\{d, T^{1/3}\log d\big\} \big)$. 
    We also develop an adaptive algorithm for the small-loss setting with regret $O(L\opt \log d + \diffp^{-1} \log^{1.5}{d})$ where $L\opt$ is the total loss of the best expert.
    Additionally, we consider DP online convex optimization in the realizable setting and propose an algorithm with near-optimal regret $\wt O \big(\diffp^{-1} d^{1.5} \big)$,
    as well as an algorithm for the smooth case with regret $\wt O \big( \diffp^{-2/3} (dT)^{1/3} \big)$, both significantly improving over existing bounds in the non-realizable regime.
\end{abstract}




==> realizable-alg-potential.tex <==

\section{Potential-based algorithm for DP-experts}
\label{sec:alg-pot}
The algorithm in~\cref{alg:SVT-zero-loss} uses the sparse vector technique to evaluate the current arm. In this section, we present a more direct algorithm that uses the sparse vector technique on a potential function. This more direct approach allows us to improve the polylogarithmic terms, which results in significant improvements for DP-OCO as we show in the next section.

We describe the algorithm in a more abstract way, which will translate more easily to OCO. Let $
\mu$ be the uniform measure over the space of experts; this will be the uniform distribution over the finite number of experts in the case of DP-OPE, and the uniform distribution over the unit ball in $\mathbb{R}^d$ in the case of DP-OCO. At a high level, the algorithm is similar to \cref{alg:SVT-zero-loss} in that it samples from the exponential mechanism, and keeps that sample until a certain condition is met. While the condition there dealt only with the chosen expert, we will instead test a global condition. For a parameter $\eta$, we define the potential $\phi_{\eta}(t) = \int \exp(-\eta \sum_{i=1}^t \ell_i(x) \mu(x) \text{d}x$. The condition we check (using the sparse vector technique) is that $\log \phi_{\eta}(t)$ has changed by at least $\alpha$ since the last resample. We formally describe the algorithm in \cref{alg:potential-experts}.


\begin{algorithm}[t]
	\caption{Potential-based Algorithm for Experts}
	\label{alg:potential-experts}
	\begin{algorithmic}[1]
		%\REQUIRE Parameters $\alpha,\bet$
		%constraint set $\xdomain$,
		%step size $\ss$, initial point $x_0$;
		\REQUIRE Switching bound $K$, Parameters $\eta, \alpha$, failure probability $\beta$, per-phase privacy parameter $\diffp_0$, measure $\mu$ on set of experts.
		\STATE Set $k=0$, $t^*(k)=0$ and sample current expert $x_0 \sim \mu$.
  
        \FOR{$t=1$ to $T$\,}
           
            \IF{$k < K$}
                \STATE $Q = \init(\diffp_0,2\alpha,\beta/T)$
                %\STATE Run a new $\AbThr$ instance over the queries $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ with privacy parameter $\diffp_0$, probability parameter $\beta/T$, accuracy parameter $\alpha$ and threshold $L=3\alpha$ 
                %\WHILE{$\AbThr$ has not halted}
                \WHILE{Q.\test() = False}
                    \STATE Set $ x_{t} =  x_{t-1}$
                    \STATE Define a new query $q_t = \frac{1}{\eta}(\log \phi_{\eta}(t^*(k)) - \log \phi_{\eta}(t))$
                    \STATE Add new query $Q.\addq(q_t)$
                    \STATE Receive loss function $\ell_t: [d] \to [0,1]$
        	        \STATE Pay cost $\ell_t(x_t)$
        	        \STATE Update $t = t+1$ %and feed a new query $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ to \AbThr
                \ENDWHILE
            
                % \STATE Run a Sparse-Vector query to identify if $\sum_{i=1}^{t-1} \ell_i(x_t) \ge \frac{100 \log(d)}{\diffp_0}$
                % \IF{Sparse-Vector identifies above threshold}
                \STATE Sample $x_t$ from the distribution:
                \begin{equation*}
                    P(x_t = x) =  e^{-\eta \sum_{i=1}^{t-1} \ell_i(x) \mu(x)} / \phi_{\eta}(t-1)
                \end{equation*}
                %\STATE Let $ x_{t}$ be the output of the exponential algorithm
                \STATE $k = k + 1$.
                \STATE $t^*(k) = t-1$.
                %\ENDIF
            \ELSE
        	\STATE Set $ x_{t} =  x_{t-1}$
        	\STATE Receive loss function $\ell_t: [d] \to [0,1]$
        	\STATE Pay cost $\ell_t(x_t)$
        	\ENDIF  
        \ENDFOR
	\end{algorithmic}
\end{algorithm}


We first observe some simple properties of $\phi_{\eta}$.
\begin{lemma}
    Suppose that the per-step losses $\ell_t(s)$ are in $[0,1]$. Then $\phi_{\eta}(t-1) \geq \phi_{\eta}(t) \geq e^{-\eta}\phi_{\eta}(t-1)$.
\end{lemma}
\begin{proof}
For any $x$, we have
\begin{align*}
\sum_{i=1}^{t-1} \ell_i(x) \leq  \sum_{i=1}^{t} \ell_i(x) \leq  \sum_{i=1}^{t-1} \ell_i(x) + 1.
\end{align*}
This implies that
\begin{align*}
e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \geq e^{-\eta \sum_{i=1}^{t} \ell_i(x)} \geq e^{-\eta} e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}. 
\end{align*}
The claim follows by integrating with respect to $\mu$.
\end{proof}

\begin{lemma}
\label{lem:svt_worked}
    Suppose that $\alpha \geq \frac{8\eta (\log T + \log 2T/\beta)}{\diffp_0}$. Then during the run of the algorithm, $\log\phi_\eta(t^*(k)) -\log\phi_\eta(t) \leq  3\alpha$ always holds except with probability $\beta$. Moreover, $\log\phi_\eta(t^*(k)) - \log\phi_\eta(t^*(k+1)) \geq \alpha$ holds for all $k$ except with probability $\beta$.    \end{lemma}
\begin{proof}
    We use sparse vector with a threshold of $2\alpha$. The condition on $\alpha$ along with the first property of the sparse vector algorithm~\cref{lemma:svt} implies that if $\log\phi_\eta(t^*) -\log\phi_\eta(t) \leq 3\alpha$. The second property of sparse vector implies the second property.
\end{proof}


We next analyze the loss of the algorithm.
\begin{lemma}
Suppose that $\eta < \frac 1 2$ and losses are in the range $[0,1]$. For some $\gamma > 0$, let $L^*(\gamma)$ be such that $\Pr_{x \sim \mu}[\sum_{t=1}^T \ell_x(t) \leq L^*(\gamma)] \geq \gamma$. Let $K \geq \frac{\eta L^*(\gamma) + \log 1/\gamma}{\alpha}$. Then the expected loss of \cref{alg:potential-experts} satisfies
\begin{align*}
    \E[\sum_{t=1}^T \ell_t(x_t)] \leq 2e^{3\alpha}(L^*(\gamma) + \frac{\log 1/\gamma}{\eta}) + 2\beta T.
\end{align*}
\end{lemma}
\begin{proof}
We first observe that by the assumption on sufficient probability mass on experts with loss at most $L^*(\gamma)$, it follows that $\phi_\eta(T) \geq \gamma e^{-\eta L^*(\gamma)}\phi_\eta(0)$. Let $E$ be the event that both the conditions on $\phi_\eta(t)$'s in ~\cref{lem:svt_worked} hold. Thus $\Pr[E] \geq 1-2\beta$. The second condition implies that if we reach the bound $K$ on the number of switches, then conditioned on $E$, $\phi_\eta(T) \leq e^{-K\alpha}\phi_\eta(0)$. Thus if $K \geq \frac{\eta L^*(\gamma) + \log 1/\gamma}{\alpha}$, then the switching bound is never reached under $E$.

    Now note that if we sampled $x \sim e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} / \phi_{\eta}(t-1)$, then we would have
    \begin{align*}
        \E[\eta\ell_t(x)/2] &= \frac{1}{\phi_{\eta}(t-1)} \int  \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \mu(x) \text{d}x\\
        & \leq \frac{1}{\phi_{\eta}(t-1)} \int  (1-e^{-\eta\ell_t(x)})e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}  \mu(x) \text{d}x\\
        & = \frac{1}{\phi_{\eta}(t-1)} \int (e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} -  e^{-\eta \sum_{i=1}^{t} \ell_i(x)}) \mu(x) \text{d}x\\
        &= \frac{\phi_{\eta}(t-1)- \phi_{\eta}(t)}{\phi_{\eta}(t-1)}\\
        &\leq \log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}.
    \end{align*}
    Here the first inequality uses the fact that for $y \in [0,1]$, we have $y/2 < 1- e^{-y}$, and the second inequality uses $(1-r) \leq -\log r$ for $r \in [\frac{1}{2},1]$. The assumptions on $\eta$ and the losses imply that the relevant conditions hold.

    Our algorithm however uses an outdated sample based on the distribution at $t^*(k)$, whenever $t$ is in phase $k$. Nevertheless, note that the cumulative losses increase with $t$ so that $e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}$ is smaller than $e^{-\eta \sum_{i=1}^{t^*(k)} \ell_i(x)}$.% Let $E$ be the event that the ratio $\frac{\phi_{\eta}(t^*(k))}{\phi_{eta}(t-1)} \leq e^{3\alpha}$. Thus $\Pr[E] \geq 1-\beta$. 
    We then write
    \begin{align*}
   \E[\eta\ell_t(x_t)/2 \cdot \mathbf{1}(E)] &= \frac{1}{\phi_{\eta}(t^*(k))} \int  \mathbf{1}(E) \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t^*(k)} \ell_i(x)} \mu(x) \text{d}x\\     &\leq \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t^*(k))}\cdot  \frac{1}{\phi_{\eta}(t-1)}\int  \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \mu(x) \text{d}x\\
        &\leq e^{3\alpha}\log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}.
    \end{align*}
Rearranging and summing over the $t$ steps, we get
    \begin{align*}
   \E[\sum_{t=1}^T\ell_t(x_t)\cdot \mathbf{1}(E)] 
           &\leq \frac{2e^{3\alpha}}{\eta} \sum_{t=1}^T\log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}\\
           &\leq \frac{2e^{3\alpha}}{\eta} \log \frac{\phi_{\eta}(0)}{\phi_{\eta}(T)}.
    \end{align*}
Since $\phi_\eta(T) \geq \gamma e^{-\eta L^*(\gamma)}\phi_\eta(0)$, we can upper bound this expression.
Furthermore, $\E[\sum_{t=1}^T\ell_t(x_t)\cdot \mathbf{1}(E^c)]$ is clearly bounded $\Pr[E^c] \cdot T \leq 2\beta T$. The claim follows.
\end{proof}

This can yield pure or approximate DP. Indeed each phase of the algorithm satisfies $(\eta + \diffp_0)$-DP. Composing over the at most $K$ phases, we get  $(\eta + \diffp_0)$-DP or $(2(\eta + \diffp_0)\sqrt{K \log 1/\delta}, \delta)$-DP. 
With this in mind, we can now plug in appropriate values of $\eta, \alpha, \eps_0$ to derive the following result for pure $\diffp$-DP.

\begin{theorem}(pure DP)
    Suppose that we run \cref{alg:potential-experts} with parameters $\alpha = 1$, $\beta = \frac{1}{T^2}$,  $K=2 \log 1/\gamma$ , $\diffp_0 = \diffp / K$, and $\eta =\diffp_0 / (56 \log T) = \diffp / (112 \log T \log 1/\gamma)$. If $L^*(\gamma) \leq \log^2 1/\gamma \log T / \diffp$, then this algorithm satisfies $\eps$-DP and incurs loss $O(L^* + \frac{\log^2 1/\gamma\log T}{\diffp})$. In particular, for DP-OPE with $d$ experts, assuming that that $OPT \leq \log^2 d \log T / \diffp$, we get regret  $O(\log^2 d \log T / \diffp)$ by setting $\gamma = \frac 1 d$.
\end{theorem}

Moreover, we have the following improved bound for \ed-DP.
\begin{theorem}(\ed-DP)
\label{thm:pot-appr}
    Suppose that for $\eps < 1$,  we run \cref{alg:potential-experts} with parameters $\alpha = 1$, $\beta = \frac{1}{T^2}$,  $K=2 \log 1/\gamma$ , $\diffp_0 = \diffp / \sqrt{K\log 1/\delta}$, and $\eta =\diffp_0 / (56 \log T) = \diffp / (112 \log T \sqrt{\log 1/\gamma\log 1/\delta})$. If $L^*(\gamma) \leq \log^{1.5} 1/\gamma \log T \sqrt{\log 1/\delta}/ \diffp$, then this algorithm satisfies $(\eps,\delta)$-DP and incurs loss $O(L^* + \frac{\log^{1.5} 1/\gamma\log T\sqrt{\log 1/\delta}}{\diffp})$. In particular, for DP-OPE with $d$ experts, assuming that $OPT \leq \log^{1.5} d \log T\sqrt{\log 1/\delta} / \diffp$, we get regret  $O(\log^{1.5} d \log T \sqrt{\log 1/\delta}/ \diffp)$ by setting $\gamma = \frac 1 d$.
\end{theorem}


For the setting of DP-OCO in the realizable case, we get that by Lipschitzness, a small ball of radius $r$ around $x^*$ has loss $O(rLT)$. Setting $r=(LT)^{-1}$ then ensures that this value is at most $1$ This ball has measure $\gamma = (r/D)^{-d}$. Scaling so that $D,L \leq 1$, 
{we get an regret $O(d^2 \log^3 T / \diffp)$ for the case of $\eps$-DP and $O(d^{1.5}\log^{2.5}  T \sqrt{\log 1/\delta}/ \diffp)$ for $(\eps,\delta)$-DP.} Finally we note that this algorithm only accesses the loss functions to sample from the exponential mechanism, and compute the potential $\phi_{\eta}(t)$. Both of these can be implemented in polynomial time for the case of $\mu$ being uniform over the ball, and the losses being convex using standard techniques from logconcave sampling. Thus this algorithm can be run in polynomial time for DP-OCO.


==> realizable-introduction.tex <==
\section{Introduction}

We study the problem of private online optimization in the realizable setting where there is a zero-loss solution. In this problem, an online algorithm $\A$ interacts with an adversary over $T$ rounds. The adversary picks a (non-negative) loss function $\ell_t: \mc{X} \to \R$ at round $t$ and simultaneously the algorithm $\A$ picks a response $x_t$, suffering loss $\ell_t(x_t)$. The algorithm aims to minimize the regret, which is the loss compared to the best solution $x\opt \in \mc{X}$ in hindsight, while at the same time keeping the sequence of predictions $x_1,\ldots,x_T$ differentially private with respect to individual loss functions. % \tk{be more precise here?}

In this paper, we focus on two well-studied instances of this problem. In differentially private online prediction from experts (DP-OPE), we have $d$ experts $\mc{X} = [d]$ and the adversary chooses a loss function $\ell_t: [d] \to [0,1]$. Our second setting is differentially private online convex optimization (DP-OCO) where $\mc{X} \subset \R^d$ is a convex set with bounded diameter, and the adversary chooses convex and $L$-Lipschitz loss functions $\ell_t : \mc{X} \to \R^+$.%\vf{$\R^+$ to make a bit more precise?}

Several papers have recently studied DP-OPE and DP-OCO in the general non-realizable setting~\cite{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17,KairouzMcSoShThXu21}. These papers have resulted in different algorithms with sub-linear regret for both problems. For DP-OPE, ~\citet{AgarwalSi17,JainTh14} developed private versions of follow-the-regularized-leader (FTRL) obtaining regret $\min\big\{ {d}/{\diffp}, {\sqrt{T \log d}}/{\diffp} \big\}$. 
More recently, \citet{AsiFeKoTa22} developed low-switching algorithms for DP-OPE with oblivious adversaries, obtaining regret roughly $O(\sqrt{T\log (d)} +  T^{1/3}\log d/ \eps)$.
Additionally, for the problem of DP-OCO, \citet{KairouzMcSoShThXu21} have recently proposed a DP-FTRL algorithm based on the binary tree mechanism which obtains regret $ \big({T\sqrt{d}}/{\diffp} \big)^{1/2}$.

Despite this progress, the regret bounds of existing algorithms are still polynomially worse than existing lower bounds. Currently, the only existing lower bounds for oblivious adversaries are the trivial bounds from the non-online versions of the same problems: for DP-OPE, lower bounds for private selection~\cite{SteinkeUll17b} imply a regret lower bound of $O({\log(d)}/{\diffp)}$, while existing lower bounds for DP-SCO~\cite{FeldmanKoTa20} give a regret lower bound of $\Omega({\sqrt{d}}/{\diffp})$ for DP-OCO.


Practical optimization problems arising from over-parameterized models often lead to instances that additionally satisfy {\em realizability}, i.e. that the optimal loss is zero or close to zero. This motivates the study of designing algorithms that can do better under this assumption.  Realizability has been studied since the early days of learning theory and ubiquitous in the non-private online optimization literature~\cite{SrebroSrTe10,Shalev12,Hazan16}.
It has proven useful for improving regret bounds in non-private OPE and OCO~\cite{Shalev12,SrebroSrTe10} and in the closely related problem of differentially private stochastic convex optimization (DP-SCO)~\cite{AsiChChDu22}.  In this work we study DP-OPE and DP-OCO in the realizable setting and develop new algorithms that obtain near-optimal regret bounds in several settings.


%Online optimization, realizable setting, 

%Gaps in private online optimization --> we close them in the realizable setting

%\cite{AroraHaKa12, Hazan16, Shalev12}

%\ha{TODO}





\subsection{Contributions}
We propose new algorithms and lower bounds %\vf{The contributions do not list any lower bounds} 
for the problems of differentially private online prediction from experts (DP-OPE) and differentially private online convex optimization (DP-OCO) in the realizable setting. The following are our primary contributions:

\begin{itemize} %[leftmargin=*]
% 
\item \textbf{Near-optimal algorithms for DP-OPE.}~~
% 
We design new algorithms that obtain near-optimal regret $\wt O \left( \log^{1.5}(d)/\diffp \right)$ for DP-OPE with $d$ experts when there is a zero-loss expert. 
The best existing algorithms for non-realizable DP-OPE obtain significantly worse regret bounds $\min\big\{{d}/{\diffp}, T^{1/3} \log d/{\diffp} \big\}$~\cite{AgarwalSi17,AsiFeKoTa22}, which have a polynomial dependence on either $T$ or the number of experts $d$.
Our algorithms build on sequential applications of the exponential mechanism to pick a good expert, and the sparse-vector-technique to identify when the current expert is no longer a good expert (with near-zero loss).  
Crucially, an oblivious adversary cannot identify which expert the algorithm has picked, resulting in a small number of switches.
We deploy a potential-based proof strategy to show that this algorithm have logarithmic number of switches.
We also show that a lower bound of $\Omega(\log d / \diffp)$ holds for any $\diffp$-DP algorithm even in the realizable case.
% 
\item \textbf{Adaptive algorithms for DP-OPE with low-loss experts.}~~
% 
We also develop an algorithm that adapts to the setting where there is an expert with low loss, that is, $L\opt = \min_{x \in [d]} \sum_{t=1}^T \ell_t(x)$. Our algorithms are adaptive to the value of $L\opt$ and obtain total regret of $L\opt \log d + \diffp^{-1} \log^{1.5} d$.
% 
\item \textbf{Near-optimal regret for low-dimensional DP-OCO.}~~
Building on our algorithms for DP-OPE, we propose a new algorithm for DP-OCO that obtains regret $\wt O \left( d^{1.5}/\diffp \right)$. This is near-optimal for low-dimensional problems where $d=O(1)$ and improves over the best existing algorithm which obtains a regret $ (T\sqrt{d}/\diffp)^{1/2}$~\cite{KairouzMcSoShThXu21}.
% 
\item \textbf{Improved regret for smooth DP-OCO.}~~
When the loss function is smooth, we show that DP-FTRL~\cite{KairouzMcSoShThXu21} with certain parameters obtains an improved regret of 
$(\sqrt{Td}/\diffp)^{2/3}$ if there is a zero-loss expert.
% 
\end{itemize}



\begin{table*}[t]
\begin{center}
    %\begin{subtable}[h]{0.8\textwidth}
		\begin{tabular}{| Sc | Sc | Sc |}
		    \hline
			  & \textbf{\darkblue{Non-realizable}} & \makecell{\textbf{\darkblue{Realizable}}\\\textbf{(This work)}}\\
			\hline
			{{\textbf{DP-OPE}}} & $\displaystyle \sqrt{{T\log d}} + A\min\left\{ \frac{\sqrt{d}}{\diffp},  \frac{T^{1/3}\log d}{\eps} \right\}$~\footnotesize{\cite{AgarwalSi17,AsiFeKoTa22}}  & $\displaystyle \frac{\log^{1.5} d}{\diffp}$ \\
			\cline{1-3} 
			\textbf{{DP-OCO}} & $\displaystyle  \left(\frac{T\sqrt{d}}{\diffp} \right)^{1/2}$~\footnotesize{\cite{KairouzMcSoShThXu21} } & $\displaystyle \frac{d^{1.5}}{\diffp}$ \\ %& $\Omega \left( \frac{d^2 }{n^2 \diffp^2}   \right)$ \\
			\cline{1-3}
			\textbf{{DP-OCO (smooth)}} & $\displaystyle  \left(\frac{T\sqrt{d}}{\diffp} \right)^{1/2}$~\footnotesize{\cite{KairouzMcSoShThXu21}} & $\displaystyle \left(\frac{\sqrt{Td}}{\diffp} \right)^{2/3}$ \\
			\hline
		\end{tabular}
    %\caption{Approximate \ed-DP.}
    %\label{fig:table-appr}
%\end{subtable}
     \end{center}
          \caption{Comparison between regret upper bounds for the realizable and non-realizable case for both DP-OPE and DP-OCO. For readability, we omit logarithmic factors in $T$ and $1/\delta$.}
     \label{tab:temps}
\end{table*}






\subsection{Related work}
Several works have studied online optimization in the realizable setting, developing algorithms with better regret bounds~\cite{Shalev12,SrebroSrTe10}. For online prediction from experts, the weighted majority algorithm obtains a regret bound of $4\log{d}$ compared to $O(\sqrt{T\log d})$ in the non-realizable setting. Moreover, for online convex optimization, \citet{SrebroSrTe10} show that online mirror descent achieves regret $4\beta D^2 + 2\sqrt{\beta D^2 T L\opt}$ compared to $O(\sqrt{T})$ in the general case.

%realizable setting~\cite{Shalev12,SrebroSrTe10}


On the other hand, the private online optimization literature has mainly studied the general non-realizable case~\cite{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17,KairouzMcSoShThXu21}.
For online prediction from experts, the best existing regret bounds for \ed-DP are $O(\diffp^{-1}\sqrt{T \log d \log(1/\delta)})$~\cite{JainTh14}  and $O(\sqrt{T\log d} + \diffp^{-1} \sqrt{d \log(1/\delta)} \log d \log^2 T)$~\cite{AgarwalSi17}. 
\citet{AsiFeKoTa22} show that these rates can be improved using a private version of the shrinking dartboard algorithm, obtaining regret roughly $O(\sqrt{T \log d} + T^{1/3} \log d/\eps)$.
For online convex optimization, \citet{KairouzMcSoShThXu21} developed a private follow-the-regularized-leader algorithm using the binary tree mechanism that obtains regret bound $\wt O\big( {T\sqrt{d}}/{\diffp} \big)^{1/2}$. %\tk{check bound here}\knote{Checked.}

The realizable setting has recently been studied in the different but related problem of differentially private stochastic convex optimization (DP-SCO)~\cite{AsiChChDu22}.  
DP-SCO and DP-OCO are closely related as one can convert an OCO algorithm into an SCO algorithm using standard online-to-batch transformations~\cite{Hazan16} %(\ha{what to cite here?}\knote{Seems fine.}). 
\citet{AsiChChDu22} study DP-SCO problems in the interpolation regime where there exists a minimizer that minimizes all loss functions, and propose algorithms that improve the regret over the general setting if the functions satisfy certain growth conditions.


%non-private realizable OCO~\cite{Shalev12}: weighted majority gets regret $4\log(d)$ for experts, and~\cite{SrebroSrTe10} gets $4\beta D^2 + 2\sqrt{\beta D^2 T L\opt}$


%online DP non-realizable~\cite{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17,KairouzMcSoShThXu21}

%DP-SCO~\cite{BassilySmTh14,BassilyFeTaTh19,FeldmanKoTa20,AsiFeKoTa21,AsiDuFaJaTa21} 

%DP-SCO with interpolation~\cite{AsiChChDu22}

==> realizable-pre.tex <==
\section{Preliminaries}
In online optimization, we have an interactive $T$-round game between an adversary and an online algorithm. In this paper, we focus on oblivious adversaries that choose in advance a sequence of loss functions $\ell_1,\dots,\ell_T$ where $\ell_t : \mc{X} \to \R$. Then, at round $t$, the adversary releases a loss function $\ell_t$ and simultaneously the algorithm plays a solution $x_t \in \mc{X}$. The algorithm then suffers loss $\ell_t(x_t)$ at this round. The regret of the online algorithm is
\begin{equation*}
    \reg_T(\A) = \sum_{t=1}^T \ell_t(x_t) - \min_{x^\star \in \mc{X}} \sum_{t=1}^T \ell_t(x^\star).
\end{equation*}
For ease of notation, for an oblivious adversary that chooses a loss sequence $\Ds = (\ell_1,\dots,\ell_T) $, we let $\A(\Ds) = (x_1,\dots,x_T)$ denote the output of the interaction between the online algorithm and the adversary.

In this work, we are mainly interested in two instances of the above general online optimization problem:

\begin{itemize} %[leftmargin=*]
\item \textbf{Online prediction from experts (OPE).}~~
% 
In this problem, we have a set of $d$ experts $\mc{X} = [d]$, and the adversary chooses loss functions $\ell_t : [d] \to [0,1]$.
% 
\item\textbf{Online convex optimization (OCO).}~~
% 
In OCO, we are optimizing over a convex set $\mc{X} \subseteq \R^d$ with bounded diameter $\diam(\mc{X}) \le D$,%
\footnote{The diameter of a set $\mc{X} \subseteq \R^d$ (in Euclidean geometry) is defined as $\diam(\mc{X}) = \sup_{x,y \in \mc{X}} \|x-y\|$.}
and the adversary chooses loss functions $\ell_t : \mc{X} \to \R$ that are convex and $L$-Lipschitz. 
\end{itemize}

We are mainly interested in the so-called realizable setting. More precisely, we say than an OPE (or OCO) problem is \emph{realizable} if there exists a feasible solution $x\opt \in \mc{X}$ such that $L\opt = \sum_{t=1}^T \ell_t(x\opt) = 0$. We also extend some of our results to the near-realizable setting where $0 < L\opt \ll T$.



The main goal of this paper is to study both of these problems under the restriction of differential privacy.

\begin{definition}[Differential Privacy]
\label{def:DP}
	A randomized  algorithm $\A$ is \emph{\ed-differentially private} against oblivious adversaries (\ed-DP) if, for all sequences $\Ds=(\ell_1,\dots,\ell_T)$ and $\Ds'=(\ell'_1,\dots,\ell'_T)$ that differ in a single element, and for all events $\cO$ in the output space of $\A$, we have
	\[
	\Pr[\A(\Ds)\in \cO] \leq e^{\eps} \Pr[\A(\Ds')\in \cO] +\delta.
	\]
\end{definition}
We note that our algorithms satisfy a stronger privacy guarantee against adaptive adversaries (see for example the privacy definition in~\cite{JainRaSiSm21}). However, we choose to focus solely on oblivious adversaries for ease of presentation and readability.



\subsection{Background on Differential Privacy}
\newcommand{\AbThr}{\ensuremath{\mathsf{AboveThreshold}}}
\newcommand{\init}{\ensuremath{\mathsf{InitializeSparseVec}}} %initialize an instance with empty set of queries
\newcommand{\addq}{\ensuremath{\mathsf{AddQuery}}} %add a new query
\newcommand{\test}{\ensuremath{\mathsf{TestAboThr}}} % test if last query is above threshold

In our analysis, we require the following standard privacy composition results.
\begin{lemma}[Basic composition~\citealp{DworkRo14}]
%\iftoggle{arxiv}{(Basic composition; \cite{DworkRo14})}
%{[Basic composition; \citealp{DworkRo14}]}
\label{lemma:basic-comp}    
    If $\A_1,\dots,A_k$ are randomized algorithms that each is $\diffp$-DP, then their composition $(\A_1(\Ds),\dots,A_k(\Ds))$ is $k \diffp$-DP.
\end{lemma}

\begin{lemma}[Advanced composition~\citealp{DworkRo14}] %add DworkRoVa10 also?
\label{lemma:advanced-comp}
    If $\A_1,\dots,A_k$ are randomized algorithms that each is $(\diffp,\delta)$-DP, then their composition $(\A_1(\Ds),\dots,A_k(\Ds))$ is $(\sqrt{2k \log(1/\delta')} \diffp + k \diffp (e^\diffp - 1),\delta' + k \delta)$-DP.
\end{lemma}


In addition to basic facts about differential privacy such as composition and post-processing, our development uses two key techniques from the privacy literature: the Sparse-vector-technique and the binary tree mechanism, which we now describe.

\paragraph{Sparse vector technique.}

We recall the sparse-vector-technique~\cite{DworkRo14} which we use for the realizable setting in~\cref{sec:upper-bounds-realizable}. Given an input $\Ds = (z_1,\dots,z_n) \in \domain^n$, the algorithm takes a stream of queries $q_1,q_2,\dots,q_T$ in an online manner. We assume that each $q_i$ is $1$-sensitive, that is, $|q_i(\Ds) - q_i(\Ds') | \le 1$ for neighboring datasets $\Ds,\Ds' \in \domain^n$ that differ in a single element.
We have the following guarantee. 
\begin{lemma}[\citealp{DworkRo14}, Theorem 3.24]
\label{lemma:svt}
    Let $\Ds = (z_1,\dots,z_n) \in \domain^n$.
    %and $\diffp \le 1$.  
    For a threshold $L$ and $\beta>0$, there is an $\diffp$-DP algorithm (\AbThr) that halts at time $k \in [T+1]$ such that for $\alpha = \frac{8(\log T + \log(2/\beta))}{\diffp}$ with probability at least $1-\beta$,
    \begin{itemize} %[nosep]
        \item For all $t < k$, $q_i(\Ds) \le L + \alpha$;
        \item $q_k(\Ds) \ge L - \alpha$ or $k = T+1$.
    \end{itemize}
\end{lemma}

To facilitate the notation for using \AbThr~in our algorithms, we assume that it has the following components:
\begin{enumerate}
    \item $\init(\diffp,L,\beta)$: initializes a new instance of \AbThr~with privacy parameter $\diffp$, threshold $L$, and probability parameter $\beta$. This returns an instance (data structure) $Q$ that supports the following two functions.
    \item $Q.\addq(q)$: adds a new query $q:\domain^n \to \R$ to $Q$.
    \item $Q.\test()$: tests if the last query that was added to $Q$ was above threshold. In that case, the algorithm stops and does not accept more queries.
\end{enumerate}

% In out algorithm, we will use sparse-vector to identify if the loss of the current expert is large. In particular, at round $t+1$, given $\ell_1,\dots,\ell_{t}$ and previous model $x_{t}$, we define the queries $q_t(\ell_1,\dots,\ell_{t}) = \sum_{j=1}^t \ell_j(x_t)$. Note that $q_t$ is a $1$-sensitive query, and therefore~\Cref{lemma:svt} with $L = 2\alpha$ implies the following result.
% \begin{lemma}~\cite[theorem 3.24]{DworkRo14}
% \label{lemma:svt-OPE}
%     Let $\diffp \le 1$ and $\ell_1,\dots,\ell_T$ be the loss functions in a DP-OPE protocol with corresponding models $x_1,\dots,x_T$.  For $\beta>0$, there is an $\diffp$-DP algorithm (\AbThr) that halts at time $k \in [T+1]$ such that for $\alpha = \frac{8(\log T + \log(2/\beta))}{\diffp}$ with probability at least $1-\beta$
%     \begin{itemize}
%         \item For all $t < k$, $\sum_{j=1}^t \ell_j(x_t) \le 3 \alpha$
%         \item For $t=k$, $\sum_{j=1}^t \ell_j(x_t) \ge \alpha$ or $k = T+1$
%     \end{itemize}
% \end{lemma}

\newcommand{\BinTr}{BinaryTree}

\paragraph{The binary tree mechanism.}

We also build on the binary tree mechanism~\cite{DworkNaPiRo10,ChanShSo11} which allows to privately estimate the running sum of a sequence of $T$ numbers $a_1,\dots,a_T \in [0,1]$. %\ha{version for vectors?}\knote{Added a sentence}
\begin{lemma}[\citealp{DworkNaPiRo10}, Theorem 4.1]
\label{lemma:bt}
    Let $\diffp \le 1$.  There is an $\diffp$-DP algorithm (\BinTr) that takes a stream of numbers $a_1,a_2,\dots,a_T$ and outputs $c_1,c_2,\dots,c_T$ such that for all $t \in [T]$ with probability at least $1-\beta$,
    \begin{equation*}
        \Big| c_t - \sum_{i=1}^t a_i \Big| 
        =
        \frac{1}{\diffp} \cdot \mathsf{poly}(\log(\beta^{-1})\log{T}).
    \end{equation*}
\end{lemma}
The same approach extends to the case when $a_i$'s are vectors in $\mathbb{R}^d$ with $\|a_i\|_2 \leq 1$. In this case, the error vector $(c_t - \sum_{i=1}^t a_i)$ is distributed at $\mathcal{N}(0, d \cdot \mathsf{poly}(\log T/\beta\delta)/\diffp^2 \mathbb{I})$ and the mechanism satisfies $(\diffp,\delta)$-DP.
%\vf{I guess polylog in this bound is really not bad so could make it explicit. And if we are going for poly then can put all in one log e.g. $poly(\log(T/\beta\delta))$. }

\paragraph{Additional notation.} 

For a positive integer $k \in \N$, we let $[k] = \{1,2,\dots,k\}$. Moreover, for a sequence $a_1,\dots,a_t$, we use the shorthand $a_{1:t} = a_1,\dots,a_t$.


==> realizable-ub-OCO.tex <==


\section{Faster rates for DP-OCO}
\label{sec:dp-oco}
In this section we study differentially private online convex optimization (DP-OCO) and propose new algorithms with faster rates in the realizable setting. In~\Cref{sec:dp-oco-experts}, we develop an algorithm that reduces the OCO problem to an experts problem (by discretizing the space) and then uses our procedure for experts. %; here, we use an improved potential-based algorithm (see~\Cref{sec:alg-pot}) for DP-OPE that improves the logarithmic dependence on the number of experts over~\cref{alg:SVT-zero-loss}. Crucially, this improves our regret for DP-OCO by polynomial factors in $d$.
In~\Cref{sec:dp-oco-smooth}, we show that follow-the-regularized-leader (FTRL) using the binary tree mechanism results in faster rates in the realizable setting for smooth functions.

\subsection{Experts-based algorithm for DP-OCO}
\label{sec:dp-oco-experts}
The algorithm in this section essentially reduces the problem of DP-OCO to DP-OPE by discretizing the space $\mc{X} = \{ x \in \R^d: \ltwo{x} \le D \}$ into sufficiently many experts. In particular, we consider a $\rho$-net of the space $\mc{X}$, that is, a set $\mc{X}_{\mathsf{experts}} = \{x^1, \dots, x^M \} \subset \mc{X}$ such that for all $x \in \mc{X}$ there is $x^i \in \mc{X}^\rho_{\mathsf{experts}}$ such that $\ltwo{x^i - x} \le \rho$. Such a set exists if $M \ge 2^{d \log(4D/\rho)}$ (\citealp{Duchi19}, Lemma 7.6). Given a loss function $\ell_t: \mc{X} \to \R$, we define the loss of expert $x^i$ to be $\ell_t(x^i)$. Then, we run~\Cref{alg:SVT-zero-loss} for the given DP-OPE problem. This algorithm has the following guarantees.

\begin{theorem}
\label{thm:DP-OCO}
    Let $\mc{X} = \{ x \in \R^d: \ltwo{x} \le D\}$
    and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be non-negative, convex and $L$-Lipschitz functions chosen by an oblivious adversary.
    %Let $\A$ be an optimal \ed-DP algorithm for DP-SCO with excess loss $O(\Delta_n)$ using $n$ samples. 
    %Then running~\Cref{alg:potential-experts} (in \Cref{sec:alg-pot}) over $\mc{X}^\rho_{\mathsf{experts}}$ with $\rho = 1/(LT\diffp)$ is \ed-DP and has regret
    Then running~\Cref{alg:SVT-zero-loss}  over $\mc{X}^\rho_{\mathsf{experts}}$ with $\rho = 1/(LT)$ is \ed-DP and with probability at least $1-O(\beta)$ has regret 
    \iftoggle{arxiv}{
    \begin{equation*}
    %   \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) 
    % \le 
        O\left( L^{\opt} d \log(LD/\beta) + \frac{d^{3/2} \log^{3/2}(LDT) \sqrt{\log(1/\delta)} + \log(T/\beta) d \log(LD/\beta)}{\diffp}  \right).
    \end{equation*} 
    }
    {
    \begin{align*}
     & \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) \right] \\
     & \le (L\opt + \frac{1}{\diffp}) d^{1.5} \cdot O\left( \mathsf{poly} (\log (DLT/\delta)) \right).
    \end{align*} 
    }
\end{theorem}
\iftoggle{arxiv}{}{We defer the proof to~\Cref{sec:proof-dp-oco}.}
\iftoggle{arxiv}{
\begin{proof}
    Let $x_1,\dots,x_T$ be the experts chosen by the algorithm.
    First, \Cref{thm:ub-realizable} implies that this algorithm obtains the following regret with respect to the best expert
    \begin{equation*}
        \sum_{t=1}^T \ell_t(x_t) - L^{\opt}_{\mathsf{experts}} \le 
        O\left( L^{\opt}_{\mathsf{experts}} \log(M/\beta) + \frac{\log^2(M) + \log(T/\beta) \log(M/\beta)}{\diffp}  \right)
        %%(L^{\opt}_{\mathsf{experts}}  + \frac{1}{\diffp}) d^{1.5} \cdot O\left( \mathsf{poly} (\log \frac{T}{\beta}) \right),
    \end{equation*}
    where $L^{\opt}_{\mathsf{experts}} = \min_{x \in \mc{X}^\rho_{\mathsf{experts}}} \sum_{t=1}^T \ell_t(x)$. Since $\ell_t$ is $L$-Lipschitz for each $t \in [T]$, we obtain that 
    \begin{equation*}
    | L\opt - L^{\opt}_{\mathsf{experts}} |
        = |\min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) - \min_{x \in \mc{X}^\rho_{\mathsf{experts}}} \sum_{t=1}^T \ell_t(x) |  
        \le T L  \rho.
    \end{equation*}
    Overall this gives
     \begin{equation*}
        \sum_{t=1}^T \ell_t(x_t) - L^{\opt} 
        \le  O\left( (L^{\opt} + TL\rho) \log(M/\beta) + \frac{\log^{3/2}(M) \sqrt{\log(1/\delta)} + \log(T/\beta) \log(M/\beta)}{\diffp}  \right).
    \end{equation*}
    Setting $\rho = 1/(LT\diffp)$ proves the claim.
\end{proof}
}

%In the realizable setting ($L\opt=0$), the normalized regret of the algorithm can be improved to $d^{1.5}/T\diffp$ (up to logarithmic factors) using \Cref{alg:potential-experts} in \Cref{sec:alg-pot}. Moreover, this algorithm runs in polynomial time. 
These results demonstrates that existing algorithms which achieve  regret roughly $(\frac{T\sqrt{d}}{ \diffp})^{1/2}$ are not optimal for the realizable setting. Moreover, in the low-dimensional regime (constant $d$), the above bound is nearly-optimal up to logarithmic factors as we have a lower bound of $\sqrt{d}/\diffp$ from the stochastic setting of this problem (see discussion in the introduction).

Finally, while the algorithm we presented in~\Cref{thm:DP-OCO} has exponential runtime due to discretizing the space, we note that applying~\Cref{alg:SVT-zero-loss} over the unit ball results in similar rates and polynomial runtime.
Recall that this algorithm only accesses the loss functions to sample from the exponential mechanism, and uses sparse-vector over the running loss. Both of these can be implemented in polynomial time---since the losses are convex---using standard techniques from log-concave sampling. 


\subsection{Binary-tree based FTRL}
\label{sec:dp-oco-smooth}
In this section, we consider DP-OCO with smooth loss functions and show that DP-FTRL~(Algorithm 1, \citealp{KairouzMcSoShThXu21}) with modified parameters obtains improved regret ${\beta D^2} + ({\sqrt{Td}}/{ \diffp})^{2/3}$ in the realizable setting, compared to ${LD}\sqrt{T} + ({T\sqrt{d}}/{ \diffp} )^{1/2}$ in the non-realizable setting.

We present the details in~\Cref{alg:dp-ftrl}. Appendix B.1 in~\cite{KairouzMcSoShThXu21} has more detailed information about the implementation of the binary tree mechanism in DP-FTRL.

\begin{algorithm}
	\caption{DP-FTRL~\cite{KairouzMcSoShThXu21}}
	\label{alg:dp-ftrl}
	\begin{algorithmic}[1]
		%\REQUIRE Data points $\Ds=(\ds_1, \ldots, \ds_n)\in \domain^n$,
		%constraint set $\xdomain$,
		%step size $\ss$, initial point $x_0$;
	\REQUIRE Regularization parameter $\lambda$	
        \STATE Set $x_0 \in \mc{X}$
        \FOR{$t=1$ to $T$\,}
            \STATE Use the binary tree mechanism to estimate the sum $\sum_{i=1}^{t-1} \nabla \ell_i(x_i)$; let $\bar g_{t-1}$ be the estimate
            \STATE Apply follow-the-regularized-leader step
            \begin{equation*}
             x_{t} = \argmin_{x \in \mc{X}} \<\bar g_{t-1}, x \> + \frac{\lambda}{2} \ltwo{x}^2,
            \end{equation*}
            \STATE Receive loss function $\ell_t: \mc{X} \to \R$
            \STATE Pay cost $\ell_t(x_t)$
        \ENDFOR
	\end{algorithmic}
\end{algorithm}


We have the following guarantees for DP-FTRL in the realizable and smooth setting. 
%\iftoggle{arxiv}{}{Due to space limitations, we prove this theorem in~\Cref{proof:dp-oco-smooth}}
\begin{theorem}
\label{thm:dp-oco-smooth}
    Let $\mc{X} = \{ x \in \R^d: \ltwo{x} \le D\}$
    and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be non-negative, convex, $L$-Lipschitz, and $\beta$-smooth functions chosen by an oblivious adversary.  DP-FTRL with $\lambda = 32 \beta + \left( \frac{\beta}{\diffp^2} (L/D)^2 T d \log(T) \log(1/\delta) \right)^{1/3}$ is \ed-DP and generates
    $x_1,\dots,x_T$ that has regret
    % \begin{equation*}
    % \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) \right]
    %     \le  \tilde O \left( L\opt +  \beta D^2 + T\left(\frac{D^2 L  \sqrt{d}}{T \diffp} \right)^{2/3} \right).
    % \end{equation*}
    \iftoggle{arxiv}{
    \begin{align*}
    \frac{1}{T} \E \left[ \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) \right]
        & \le  O \left( \frac{L\opt +  \beta D^2}{T} +  \left(  LD \frac{ \sqrt{\beta D^2 d \log(T) \log(1/\delta)}}{T \diffp} \right)^{2/3}  \right).
    \end{align*}
    }
    {
    \begin{align*}
    &  \E \left[ \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) \right] \\
        & \le  O \left( {L\opt +  \beta D^2} +  \left(  LD \frac{ \sqrt{\beta D^2 T d \log(T) \log(1/\delta)}}{ \diffp} \right)^{2/3}  \right).
    \end{align*}
    }
\end{theorem}
%\iftoggle{arxiv}{
For the proof, we use the following property for smooth non-negative functions.
%\begin{lemma}[\citealp{SrebroSrTe10}, Lemma 2.1]
\begin{lemma}[\citealp{Nesterov04}]
    Let $\ell: \mc{X} \to \R$ be non-negative and $\beta$-smooth function. Then $\ltwo{\nabla \ell(x)}^2\le 4 \beta \ell(x)$.
\end{lemma}
\begin{proof}
    The proof follows similar arguments to the proof of Theorem 5.1 in~\cite{KairouzMcSoShThXu21}. Let 
    \begin{equation*}
        x_{t+1} = \argmin_{x \in \mc{X}} \sum_{i=1}^t \<\nabla \ell_i(x_i), x \> + \frac{\lambda}{2} \ltwo{x}^2 + \<b_t,x\>,
    \end{equation*}
    be the iteration of DP-FTRL where $b_t$ is the noise added by the binary tree mechanism. Moreover, let $\hat x_{t+1}$ be the non-private solution, that is, 
    \begin{equation*}
        \hat x_{t+1} = \argmin_{x \in \mc{X}} \sum_{i=1}^t \<\nabla \ell_i(x_i), x \> + \frac{\lambda}{2} \ltwo{x}^2 .
    \end{equation*}
    Lemma C.2 in~\cite{KairouzMcSoShThXu21} states that $\ltwo{x_{t+1} - \hat x_{t+1}} \le \ltwo{b_t}/\lambda$. Therefore, we have
    \iftoggle{arxiv}{
    \begin{align*}
    \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) 
        & \le \sum_{t=1}^T  \< \nabla \ell_t(x_t), x_t - x\opt\> \\
        & = \sum_{t=1}^T  \< \nabla \ell_t(x_t), x_t - \hat x_t\> + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\
        & \le \sum_{t=1}^T \ltwo{\nabla \ell_t(x_t)} \ltwo{x_t - \hat x_t} + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\ 
        & \le \frac{1}{8 \beta} \sum_{t=1}^T \ltwo{\nabla \ell_t(x_t)}^2 +  4\beta \sum_{t=1}^T\ltwo{x_t - \hat x_t}^2 + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\ 
        & \le \frac{1}{2} \sum_{t=1}^T \ell_t(x_t) +  4 \beta \sum_{t=1}^T \ltwo{b_t}^2/\lambda^2 + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\>,
    \end{align*}
    }
    {
    \begin{align*}
    & \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) \\
        & \le \sum_{t=1}^T  \< \nabla \ell_t(x_t), x_t - x\opt\> \\
        & = \sum_{t=1}^T  \< \nabla \ell_t(x_t), x_t - \hat x_t\> + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\
        & \le \sum_{t=1}^T \ltwo{\nabla \ell_t(x_t)} \ltwo{x_t - \hat x_t} + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\ 
        & \le \frac{1}{8 \beta} \sum_{t=1}^T \ltwo{\nabla \ell_t(x_t)}^2 +  4\beta \sum_{t=1}^T\ltwo{x_t - \hat x_t}^2  \\
        & \quad + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \\ 
        & \le \frac{1}{2} \sum_{t=1}^T \ell_t(x_t) +  4 \beta \sum_{t=1}^T \ltwo{b_t}^2/\lambda^2 \\
        & \quad + \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\>,
    \end{align*}
    
    }
    where the second inequality follows from the Fenchel-Young inequality.
    % Moreover, standard results for non-private FTRL give the upper bound $\sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> \le \frac{T L^2}{\lambda} + \frac{\lambda D^2}{2} $. Overall, as $\ltwo{b_t} \le \sigma \sqrt{d \log(T) \log(T/\alpha)}$ with probability at least $1-\alpha$, we have
    % \begin{align*}
    % \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) 
    %     & \le 2 \beta \sum_{t=1}^T \ell_t(x_t) +  \frac{T \sigma^2 {d \log(T) \log(T/\alpha)}}{2 \lambda^2} + \frac{T L^2}{\lambda} + \frac{\lambda D^2}{2}.
    % \end{align*}    
    % As $\beta \le 1/4$ and $\sigma^2 \approx L^2/\diffp^2$, setting $\lambda = \frac{L \sqrt{T}}{D} + \left( T \sigma^2 d \log(T)\log(T/\alpha)/D^2 \right)^{1/3}$, this shows that 
    % \begin{align*}
    % \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) 
    %     & \le  O \left(L\opt +  LD \sqrt{T} +  \left(D^4 L^2 T d \log(T) \log(T/\alpha)/\diffp^2 \right)^{1/3}  \right).
    % \end{align*}  \\
    We can now upper bound the right term. Indeed, Theorem 5.2 in~\cite{Hazan16} implies that FTRL has 
    \begin{align*}
        \sum_{t=1}^T  \< \nabla \ell_t(x_t), \hat x_t - x\opt\> & \le \frac{2}{\lambda} \sum_{t=1}^T \ltwo{\nabla \ell_t(x_t)}^2 + \lambda D^2 \\
        & \le \frac{8 \beta}{\lambda} \sum_{t=1}^T \ell_t( x_t)  + \lambda D^2.
    \end{align*}
    Overall we now get 
    \iftoggle{arxiv}{
    \begin{align*}
    \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) 
        & \le \frac{1}{2} \sum_{t=1}^T \ell_t(x_t) +  \frac{4\beta }{ \lambda^2} \sum_{t=1}^T \ltwo{b_t}^2  
        + \frac{8 \beta}{\lambda} \sum_{t=1}^T \ell_t( x_t)  + \lambda D^2.
    \end{align*}  
    }
    {
    \begin{align*}
    \sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) 
        & \le \frac{1}{2} \sum_{t=1}^T \ell_t(x_t) +  \frac{4\beta }{ \lambda^2} \sum_{t=1}^T \ltwo{b_t}^2  \\
        & + \frac{8 \beta}{\lambda} \sum_{t=1}^T \ell_t( x_t)  + \lambda D^2.
    \end{align*}  
    
    }
    The binary tree mechanism also guarantees that for all $t \in [T]$, $$\E[\ltwo{b_t}^2] \le O \left( \frac{L^2 d \log(T) \log(1/\delta)}{\diffp^2} \right)$$ (see Appendix B.1 in~\cite{KairouzMcSoShThXu21}).
    Thus, taking expectation and setting the regularization parameter to $\lambda = 32 \beta + \big( \frac{\beta}{\diffp^2} (L/D)^2 T d \log(T) \log(1/\delta) \big)^{1/3}$, we have
    \iftoggle{arxiv}{
    \begin{align*}
    \E \left[\sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) \right]
        & \le  O \left(L\opt +  \beta D^2 +  \left( \beta D^2 (LD)^2 \frac{T d \log(T) \log(1/\delta)}{\diffp^2} \right)^{1/3}  \right).
    \end{align*} 
    }
    {
    \begin{align*}
    & \E \left[\sum_{t=1}^T \ell_t(x_t) - \ell_t(x\opt) \right] 
         \le  O (L\opt +  \beta D^2 ) \\
         & \quad + O\left( \left( \beta D^2 (LD)^2 \frac{T d \log(T) \log(1/\delta)}{\diffp^2} \right)^{1/3}  \right).
    \end{align*} 
    
    }
\end{proof}
%}

    




==> realizable-ub-experts.tex <==




% \iftoggle{arxiv}{}
% {
% % \section{Preliminaries for the realizable setting}
% % In this section, we recall existing results on sparse-vector-technique and the binary tree mechanism which we use in the realizable setting (\cref{sec:upper-bounds-realizable}).

% \section{Background on differential privacy}
% We recall the following preliminary results on differential privacy which we use in our proofs.
% \begin{lemma}
% \label{lemma:adv-comp}
%     Let $T \in \N$ and $ \Fl = \{\ell \mid  \ell : [d] \to [0,1]\}$ be the space of loss functions.
%     Let $\A_t : \Fl^t \times [d]^{t-1} \to [d]$ be $\diffp_t$-DP. Then for any $\delta>0$, their composition is $(\diffp,\delta)$-DP where
%     \begin{equation*}
%         \diffp = \frac{3}{2} \sum_{t=1}^T \diffp_t^2 + \sqrt{6 \sum_{t=1}^T \diffp_t^2 \log(1/\delta) }.
%     \end{equation*}
% \end{lemma}


% \newcommand{\AbThr}{AboveThreshold}
% \newcommand{\init}{InitializeSparseVec} %initialize an instance with empty set of queries
% \newcommand{\addq}{AddQuery} %add a new query
% \newcommand{\test}{TestAboThr} % test if last query is above threshold


% \subsection{Sparse vector technique}
% In this section, we recall the sparse-vector-technique~\cite{DworkRo14} which we use for the realizable setting in~\cref{sec:upper-bounds-realizable}. Given an input $\Ds = (z_1,\dots,z_n) \in \domain^n$, the algorithm takes a stream of queries $q_1,q_2,\dots,q_T$ in an online manner. We assume that each $q_i$ is $1$-sensitive, that is, $|q_i(\Ds) - q_i(\Ds') | \le 1$ for neighboring datasets $\Ds,\Ds' \in \domain^n$ that differ in a single element.
% We have the following guarantee. 
% \begin{lemma}~\cite[theorem 3.24]{DworkRo14}
% \label{lemma:svt}
%     Let $\Ds = (z_1,\dots,z_n) \in \domain^n$.
%     %and $\diffp \le 1$.  
%     For a threshold $L$ and $\beta>0$, there is an $\diffp$-DP algorithm (\AbThr) that halts at time $k \in [T+1]$ such that for $\alpha = \frac{8(\log T + \log(2/\beta))}{\diffp}$ with probability at least $1-\beta$
%     \begin{itemize}
%         \item For all $t < k$, $q_i(\Ds) \le L + \alpha$
%         \item $q_k(\Ds) \ge L - \alpha$ or $k = T+1$
%     \end{itemize}
% \end{lemma}

% To facilitate the notation for using \AbThr~in our algorithms, we assume that it has the following components:
% \begin{enumerate}
%     \item $\init(\diffp,L,\beta)$: initializes a new instance of \AbThr~with privacy parameter $\diffp$, threshold $L$, and probability parameter $\beta$. This returns an instance (data structure) $Q$ that supports the following two functions.
%     \item $Q.\addq(q)$: adds a new query $q:\domain^n \to \R$ to $Q$.
%     \item $Q.\test()$: tests if the last query that was added to $Q$ was above threshold. In that case, the algorithm stops and does not accept more queries.
% \end{enumerate}


% \newcommand{\BinTr}{BinaryTree}

% \subsection{The binary tree mechanism}
% We also build on the binary tree mechanism~\cite{DworkNaPiRo10,ChanShSo11} which allows to privately estimate the running sum of a sequence of $T$ numbers $a_1,\dots,a_T \in [0,1]$.
% \begin{lemma}~\cite[theorem 4.1]{DworkNaPiRo10}
% \label{lemma:svt}
%     Let $\diffp \le 1$.  There is an $\diffp$-DP algorithm (\BinTr) that takes a stream of numbers $a_1,a_2,\dots,a_T$ and outputs $c_1,c_2,\dots,c_T$ such that for all $t \in [T]$ with probability at least $1-\beta$
%     \begin{equation*}
%         |c_t - \sum_{i=1}^t a_i| \le O \left( \frac{\mathsf{poly}(\log T/\beta)}{\diffp} \right).
%     \end{equation*}
% \end{lemma}
% }


\section{Near-optimal regret for online prediction from experts}
\label{sec:upper-bounds-realizable}
In this section, we consider the online prediction from experts problem in the near-realizable regime,
% move beyond the worst-case setting of prior results and consider oblivious adversaries,
where the best expert achieves small loss $L\opt ll T$. 
Under this setting, 
% where the best experts obtains loss $\min_{x\in[d]} \sum_{t=1}^T \ell_t(x) \le L\opt$, 
we develop a new private algorithm that achieves regret $\wt O(L\opt \log d + \log^{3/2}(d)/\diffp)$. For the realizable setting where $L\opt=0$, this algorithm obtains near-optimal regret $\wt O(\log^{3/2} (d)/\diffp)$. %These results resemble recent improvements in the related problem of differentially private stochastic convex optimization (DP-SCO) where interpolation problems---where there is a model that has zero loss---exhibit faster rates than non-interpolation problems~\cite{AsiChChDu22}.

The algorithm builds on the fact that an oblivious adversary cannot know which expert the algorithm picks. Therefore, if the algorithm picks a random good expert with loss smaller than $L\opt$, the adversary has to increase the loss for many experts before identifying the expert chosen by the algorithm. The algorithm will therefore proceed as follows:
at each round, privately check using sparse-vector-technique whether the previous expert is still a good expert (has loss nearly $L\opt$). If not, randomly pick (privately) a new expert from the set of remaining good experts. The full details are in~\cref{alg:SVT-zero-loss}. 

The following theorem summarizes the performance of~\cref{alg:SVT-zero-loss}. 
\begin{theorem}
\label{thm:ub-realizable}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary such that there is $x\opt \in [d]$ such that $\sum_{t=1}^T \ell_t(x\opt) \le L\opt$. Let $0 < \beta < 1/2$, $B = \log(2T^2/\beta)$, and $L = L\opt + 4/\eta + \frac{8B}{\diffp}$. If $\eta = \diffp/(12\ceil{\log d} +  48 \log(1/\beta)) $ then
    \cref{alg:SVT-zero-loss} is $\diffp$-DP and with probability at least $1-O(\beta)$ has regret 
    \iftoggle{arxiv}{
    \begin{equation*}
        \sum_{t=1}^T \ell_t(x_t) \le O\left( L\opt \log(d/\beta) + \frac{\log^2(d) + \log(T/\beta) \log(d/\beta)}{\diffp}  \right).
    \end{equation*}
    }
    {
    \begin{align*}
     & \sum_{t=1}^T \ell_t(x_t) 
      \le O\left( L\opt \log(d/\beta) \right) \\
      & \quad + O\left( \frac{\log^2(d) + \log(T/\beta) \log(d/\beta)}{\diffp}  \right).
    \end{align*}
    }
    Further, if $\diffp \le  \sqrt{\log T \log(1/\delta)}$ and $\eta = \diffp/\sqrt{32(6\ceil{\log d} +  24 \log(1/\beta)) \log(1/\delta)}$ then
    \cref{alg:SVT-zero-loss} is $(\diffp,\delta)$-DP and with probability at least $1-O(\beta)$ has regret 
    \iftoggle{arxiv}{
    \begin{equation*}
        \sum_{t=1}^T \ell_t(x_t) \le O\left( L\opt \log(d/\beta) + \frac{\log^{3/2}(d)\sqrt{\log(1/\delta)} + \log(T/\beta) \log(d/\beta)}{\diffp}  \right).
    \end{equation*}
    }
    {
    \begin{align*}
     & \sum_{t=1}^T \ell_t(x_t) 
     \le O\left( L\opt \log(d/\beta) \right)\\ & \quad  + O \left( \frac{\log^{3/2}(d)\sqrt{\log(1/\delta)} + \log(T/\beta) \log(d/\beta)}{\diffp}  \right).
    \end{align*}
    }
\end{theorem}
% 
While \cref{alg:SVT-zero-loss} requires the knowledge of $L\opt$, we also design an adaptive version that does not require $L\opt$ in the next section. Note that the algorithm obtains regret roughly $\log^{3/2} (d)/\diffp$ for the realizable setting where $L\opt = 0$. 






\begin{algorithm}[t]
	\caption{Sparse-Vector for zero loss experts }
	\label{alg:SVT-zero-loss}
	\begin{algorithmic}[1]
		%\REQUIRE Parameters $\alpha,\bet$
		%constraint set $\xdomain$,
		%step size $\ss$, initial point $x_0$;
		\REQUIRE Switching bound $K$, optimal loss $L\opt$, Sampling parameter $\eta$, Threshold parameter $L$, failure probability $\beta$, privacy parameters $(\diffp,\delta)$
		\STATE Set $K = 6\ceil{\log d} +  24 \log(1/\beta)$, $k=0$, and current expert $x_0 = \mathsf{Unif}[d]$	
        \STATE Set $t_p = 0$
        \WHILE{$t \le T$\,}
            \STATE Set $ x_{t} =  x_{t-1}$
            \IF{$k < K$}
                \STATE $Q = \init(\diffp/2,L,\beta/T)$
                %\STATE Run a new $\AbThr$ instance over the queries $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ with privacy parameter $\diffp_0$, probability parameter $\beta/T$, accuracy parameter $\alpha$ and threshold $L=3\alpha$ 
                %\WHILE{$\AbThr$ has not halted}
                \WHILE{Q.\test() = False}
                    \STATE Set $ x_{t} =  x_{t-1}$
                    \STATE Define a new query $q_t = \sum_{i=t_p}^{t-1} \ell_i(x_t)$
                    \STATE Add new query $Q.\addq(q_t)$
                    \STATE Receive loss function $\ell_t: [d] \to [0,1]$
        	        \STATE Pay cost $\ell_t(x_t)$
        	        \STATE Update $t = t+1$ %and feed a new query $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ to \AbThr
                \ENDWHILE
            
                % \STATE Run a Sparse-Vector query to identify if $\sum_{i=1}^{t-1} \ell_i(x_t) \ge \frac{100 \log(d)}{\diffp_0}$
                % \IF{Sparse-Vector identifies above threshold}
                \STATE Sample $x_t$ from the exponential mechanism with scores $s_t(x) = \max \left(\sum_{i=1}^{t-1} \ell_i(x),L\opt \right)$ for $x \in [d]$:
                \begin{equation*}
                    \P(x_t = x) \propto e^{-\eta s_t(x)/2 }
                \end{equation*}
                %\STATE Let $ x_{t}$ be the output of the exponential algorithm
                \STATE Set $k = k + 1$ and $t_p = t$
                %\ENDIF
            \ENDIF
            \STATE Receive loss function $\ell_t: [d] \to [0,1]$
            \STATE Pay cost $\ell_t(x_t)$ 
            \STATE Update $t = t+1$
        \ENDWHILE
	\end{algorithmic}
\end{algorithm}


\begin{proof}
First, we prove the privacy guarantees of the algorithm using privacy composition results: there are $K$ applications of the exponential mechanism with privacy parameter $\eta$. Moreover, sparse-vector is applied over each user's data only once, hence the $K$ applications of sparse-vector are $\diffp/2$-DP. Overall, the algorithm is $(\diffp/2 + K\eta)$-DP and $(\diffp/2 + \sqrt{2K \log(1/\delta)} \eta + K \eta (e^\eta - 1),\delta)$-DP (using advanced compositions; see~\Cref{lemma:advanced-comp}). Setting $\eta = \diffp/2K$ results in $\diffp$-DP and $\eta = O(\diffp/\sqrt{K \log(1/\delta)})$ results in \ed-DP.

We proceed to analyze utility. First, note that the guarantees of the sparse-vector algorithm (\Cref{lemma:svt}) imply that with probability at least $1-\beta$ for each time-step $t \in [T]$, if sparse-vector identifies above threshold query then $s_t(x) \ge \ubar \Delta \defeq L - \frac{8B}{\diffp} \ge 4/\eta$. Otherwise, $s_t(x) \le \bar \Delta \defeq L + \frac{8B}{\diffp}$. In the remainder of the proof, we condition on this event. The idea is to show that the algorithm has logarithmic number of switches, and each switch the algorithm pays roughly $1/\diffp$ regret.
\\
To this end, we define a potential at time $t \in [T]$:
\begin{equation*}
    \phi_t = \sum_{x \in [d]} e^{-\eta L_t(x)/2} ,
\end{equation*}
where $L_t(x) = \max( \sum_{j=1}^{t-1} \ell_j(x), L\opt)$.
Note that $\phi_1 = d e^{-\eta L\opt/2}$ and $\phi_t \ge e^{-\eta L\opt/2}$ for all $t \in [T]$ as there is $x \in [d]$ such that $\sum_{t=1}^T \ell_t(x) = L\opt$.
We split the iterates to $m = \ceil{\log d}$ rounds $t_0,t_1,\dots,t_m$ where $t_i$ is the largest $t\in[T]$ such that $\phi_{t_i} \ge \phi_1/2^{i}$. 
Let $Z_i$ be the number of switches in $[t_i,t_{i+1}-1]$ (number of times the exponential mechanism is used to pick $x_t$).
The following key lemma shows that $Z_i$ cannot be too large.
\begin{lemma}
\label{lemma:prob-switch}
    Fix $0 \le i \le m-1$. Then for any $1 \le k \le T$, it holds that
    \begin{equation*}
        P(Z_i = k+1) \le (2/3)^k.
    \end{equation*}
\end{lemma}
\begin{proof}
Let $t_i \le t \le t_{i+1}$ be a time-step where a switch happens (exponential mechanism is used to pick $x_{t}$). Note that $\phi_{t_{i+1}} \ge \phi_{t}/2$. We prove that the probability that $x_t$ is switched between $t$ and $t_{i+1}$ is at most $2/3$. To this end, note that if $x_t$ is switched before $t_{i+1}$ then $\sum_{i=t}^{t_{i+1}} \ell_i(x) \ge \ubar \Delta$ as sparse-vector identifies $x_t$, and therefore $L_{t_{i+1}}(x) - L_t(x) \ge \ubar \Delta - L\opt \ge 4/\eta$. %(as it may be the case that $L_t(x) = L\opt \le \sum_{i=1}^{t} \ell_i(x)$). 
Thus we have that
\iftoggle{arxiv}{
\begin{align*}
P(x_{t} \text{ is switched before $t_{i+1}$})
    & \le \sum_{x \in [d]} P(x_t=x) \indic{L_{t_{i+1}}(x) - L_t(x) \ge 4/\eta} \\
    & = \sum_{x \in [d]} \frac{e^{-\eta L_{t}(x)/2}}{\phi_{t}}\cdot \indic{L_{t_{i+1}}(x) - L_t(x) \ge 4/\eta } \\
    & \le \sum_{x \in [d]} \frac{e^{-\eta L_{t}(x)/2}}{\phi_{t}}\cdot \frac{1 - e^{-\eta (L_{t_{i+1}}(x)- L_t(x))/2}}{1 - e^{-2} } \\
    & \le 4/3 (1 - \phi_{t_{i+1}}/\phi_{t}) \\
    & \le 2/3.
\end{align*}
}
{
\begin{align*}
& P(x_{t} \text{ is switched before $t_{i+1}$}) \\
    & \le \sum_{x \in [d]} P(x_t=x) \indic{L_{t_{i+1}}(x) - L_t(x) \ge 4/\eta} \\
    & = \sum_{x \in [d]} \frac{e^{-\eta L_{t}(x)/2}}{\phi_{t}}\cdot \indic{L_{t_{i+1}}(x) - L_t(x) \ge 4/\eta } \\
    & \le \sum_{x \in [d]} \frac{e^{-\eta L_{t}(x)/2}}{\phi_{t}}\cdot \frac{1 - e^{-\eta (L_{t_{i+1}}(x)- L_t(x))/2}}{1 - e^{-2} } \\
    & \le 4/3 (1 - \phi_{t_{i+1}}/\phi_{t}) \\
    & \le 2/3.
\end{align*}
}
where the second inequality follows the fact that $\indic{a \ge b} \le \frac{1-e^{-\eta b}}{1 - e^{-\eta a}}$ for $a,b,\eta \ge 0$, 
%the third inequality follows since $\eta \ubar \Delta  \ge 4$, 
and the last inequality since $\phi_{t_{i+1}}/\phi_{t_1} \ge 1/2$.
This argument shows that after the first switch inside the range $[t_i,t_{i+1}]$, each additional switch happens with probability at most $2/3$. The claim follows.
\end{proof}

We now proceed with the proof. Let $Z = \sum_{i=0}^{m-1} Z_i$ be the total number of switches. 
Note that $Z \le m + \sum_{i=0}^{m-1} \max(Z_i-1,0)$ and \Cref{lemma:prob-switch} implies $\max(Z_i-1,0)$ is upper bounded by a geometric random variable with success probability $1/3$. Therefore, using concentration of geometric random variables (\Cref{lemma:geom-concentration}), we get that
\begin{equation*}
 P(Z \ge  6m + 24 \log(1/\beta) ) \le \beta . 
\end{equation*}
% as the probability of each additional switch (after $m$ switches) is at most $2/3$. This shows that
% \begin{equation*}
%     P(Z > \ceil{\log d} + C\log T/\beta) 
%     \le T (2/3)^{C\log T/\beta} 
%     \le T (1/2)^{C/2\log T/\beta} \le \beta,
% \end{equation*}
% by setting $C = 2$. 
Noting that $K \ge 6m + 24 \log(1/\beta)$, this shows that the algorithm does not reach the switching budget with probability $1-O(\beta)$. Thus, the guarantees of the sparse-vector algorithm imply that the algorithm pays regret at most $\bar \Delta$ for each switch, hence the total regret of the algorithm is at most $O(\bar \Delta (m + \log(1/\beta))) = O(\bar \Delta \log(d/\beta)) $. The claim follows as $\bar \Delta \le L\opt + 4/\eta + 16B/\diffp$.
\end{proof}

\begin{comment}

\newcommand{\Sg}{S_{\mathsf{good}}}
\newcommand{\Sb}{S_{\mathsf{bad}}}
\newcommand{\Sc}{S_{\mathsf{chosen}}}

\begin{proof}
    The algorithm consists of at most $K$ applications of \AbThr{} and the exponential mechanism. As \AbThr{} is $\diffp_0$-DP and the exponential mechanism is $\diffp_0$-DP as well (since $s_t(x)$ is $1$-sensitive function), the final mechanism is $2K\diffp_0$-DP.
    
    Now we prove utility. Let $k$ be the number of switches that the algorithm makes, that is, the number of queries on which sparse-vector finds an above threshold query. Let $\alpha = \frac{B}{\diffp_0}$ and define a set of good experts $ \Sg^t= \{x \in[d] : \sum_{i=1}^{t-1} \ell_i(x) \le L\opt  + \alpha \}$ and a set of bad experts $\Sb^t = [d] \setminus \Sg^t$. First, note that the guarantees of \AbThr{} (\Cref{lemma:svt}) imply that with probability at least $1-\beta$, for all $t \in [T]$ where \AbThr{} halts (that is, a switch happens), we have that $\sum_{i=1}^{t-2} \ell_i(x_{t-2}) \le L\opt +  4 \alpha$ and $\sum_{i=1}^{t-1} \ell_i(x_{t-1}) \ge L\opt + 2 \alpha$. This means that $x_{t-1} \notin \Sg^t$ when \AbThr{} makes a switch. 
    Moreover, %let $ \Sc^t= \{x \in[d] : \sum_{i=1}^{t-1} \ell_i(x) \le \min_{x \in [d]} \sum_{i=1}^{t-1} \ell_i(x)  + \alpha \}$ be the set of near-optimal experts at time $t$. 
    the exponential mechanism picks $x_t$ such that $\P(x_t \notin \Sg^t) \le d e^{-\alpha \diffp_0} \le d e^{-B} \le \beta/T$. Thus, with probability at least $1-\beta$, for all $x_t$ picked by the exponential mechanism, we have $x_t \in \Sg^t$.
    Thus, we now assume that these two events happen and proceed to finish the proof conditioning on that.
    
    We will prove that if there exists an expert with loss $\sum_{t=1}^T \ell_t(x) = L\opt$, then $\P(k > K) < \beta$. Note that this will prove the claim as the regret of the algorithm in this case is at most $K (L\opt + 4\alpha)$ since \AbThr{} guarantees that the model at each switch has cumulative loss at most $L\opt + 4\alpha$. The proof will go as follows: %we will have a set of good experts  $ \Sg^t= \{x \in[d] : \sum_{i=1}^t \ell_i(x) \le \alpha \}$ and a set of bad experts $\Sb^t = [d] \setminus \Sg^t$. The main idea is to 
    we show that the adversary has to shrink the size of $\Sg^t$ by a constant factor every $O(\mathsf{poly}(B))$ switches and therefore after $k = O(\mathsf{poly} (B))$ switches the set $\Sg^t$ has only one expert (which has small loss) which will be chosen by the exponential mechanism with high probability.
    
   
    
    
    %To this end, let $B = 1/\diffp$ denote the block length and let $B_1,\dots,B_m$ denote the blocks where $m = n/B$. 
    Recall that $s_t(x) = \max(\sum_{i=1}^{t-1} \ell_i(x),L\opt)$.
    We write the set $\Sg^t$ as the union of the sets $S^t_j$ for $1 \le j \le B$ where 
    \begin{equation*}
        S^t_j = \left\{ x\in[d]: \frac{j-1}{\diffp_0} \le s_t(x) - L\opt \le \frac{j}{\diffp_0} \right\}.
    \end{equation*}
    Crucially, each set $S^t_j$ contains experts that are almost indistinguishable by a private algorithm and therefore the exponential mechanism will assign similar probabilities for experts in the same set. Let $N^t_j = |S^t_j|$. We have the following lemma.
    \begin{lemma}
        \label{lemma:switching-shrinkage}
        Assume the algorithms makes a switch at times $t_1 < t_2$. Then
        there is $\hat j \in [B]$ such that with probability $\frac{1}{12 B}$ we have
        \begin{equation*}
            \sum_{j=1}^{\hat j} N^{t_2}_j \le \left(1-\frac{1}{4B}\right) \sum_{j=1}^{\hat j} N^{t_1}_j .
        \end{equation*}
    \end{lemma}
    \noindent
    Assuming correctness of~\cref{lemma:switching-shrinkage} for now, we proceed to prove that $k<K$ with high probability. Assume we have $k$ switches at time-steps $t_1,t_2,\dots,t_k$. Let $\hat j_i \in [B]$ be the corresponding $\hat j$ from~\cref{lemma:switching-shrinkage} at time-step $t_i$. Assume that  $k > K/2 \ge 200B^2\log(d/\beta)$. Then there is a $\hat j \in [B]$ that appears at least $K/2B$ times. Noting that the sum $\sum_{j=1}^{\hat j} N^{t}_j$ cannot increase, \cref{lemma:switching-shrinkage} now implies that at time $t_k +1$ we have with probability at least $1-\beta$ (Chernoff inequality. See~\cref{lemma:chernoff})
    \begin{align*}
        \sum_{j=1}^{\hat j} N^{t_k}_j 
        &\le \max \left( \left(1-\frac{1}{4B}\right)^{K/48B} \sum_{j=1}^{\hat j} N^{1}_j,1 \right)
        \\
        &\le \max \left(e^{-K/200B^2}  d,1 \right)
        = 1.
    \end{align*}
    As we know that there is an expert with loss $\sum_{i=1}^{T} \ell_i(x) = L\opt$, this shows that $|\Sg^{t_k}| = 1$ and therefore sparse-vector will not do any more switches. This proves the claim.
    % 
    %As $p \ge 1$ and there is a zero loss expert, this establishes that $N^{t_k+1}_1 =1$. Now we have two cases. In the first, the probability of the exponential mechanism to return the zero loss expert is larger than $1/2$ which implies that after $k=5 \log d$ switches the algorithm will have picked the zero-loss expert with high probability. Otherwise, assume the probability is less than $1/2$. Similar application of~\cref{lemma:switching-shrinkage} \hac{prove general lemma for this} implies now that for some $p \ge 2$ we have after $k \ge 200 \log^4 d$
    %\begin{equation*}
    %    \sum_{i=1}^p N^{t_k+1}_i \le 1.
    %\end{equation*}
    %Since $p \ge 2$ and $N^{t}_1 \ge 1$ for all $t$, we have that $N^t_2 = 0$. Repeating the above process for $2 \log d$ times, we have that after $O(\log^5 d)$ switches $N^t_i = 0$ for $2 \le i \le 2 \log d$ and therefore the algorithm will pick the zero-loss expert with high probability. This finishes the proof.
\end{proof}



Now we proceed to prove~\cref{lemma:switching-shrinkage}. The following lemma shows that if the exponential mechanism chooses an expert from $S^t_j$ then the adversary has to eliminate roughly $N^t_j/2$ experts from $S^t_j$ (move them to $\Sb$) in order to force a switch.
\begin{lemma}
\label{lemma:adv-eliminiation}
        Assume the exponential mechanism chooses an expert $x_{t_1} \in S^{t_1}_j$ at time $t_1$. Let $t_2$ be the time of the next switch that the algorithm makes. Then with probability $1/6$ we have
        \begin{equation*}
         |  S^{t_1}_j \cap \Sg^{t_2} | \le \frac{N^{t_1}_j}{2}.
        \end{equation*}
\end{lemma}

\begin{proof}
    We analyze a stronger adversary that knows the switching times and the set $S^{t_1}_j$ from which the expert was chosen. We show that even such an adversary has to eliminate a constant fraction of the experts in $S^{t_1}_j$ before enforcing the algorithm to make a switch. To this end, %let $p_x = p(x_{t_1}=x)$ for $x \in [d]$ and 
    note that for each $x_1,x_2 \in S^{t_1}_j$ we have
    \begin{equation*}
    e^{-1} \le  \frac{\P(x_{t_1}=x_1)}{\P(x_{t_1}=x_2)} \le e.
    \end{equation*}
    Therefore we have that for all $x \in S^{t_1}_j$
    \begin{equation*}
    \frac{1}{e N^{t_1}_j} \le \P(x_{t_1}=x \mid x_{t_1} \in S^{t_1}_j) \le \frac{e}{ N^{t_1}_j}.
    \end{equation*}
    Note that for the adversary to enforce the algorithm to make a switch at time $t_2$, the guarantees of \AbThr~imply that the loss of $x_{t_1}$ must satisfy $\sum_{i=1}^{t_2-1} \ell_i(x_{t_1}) \ge L\opt + 2\alpha $ (and hence $x_{t_1} \notin \Sg^{t_2}$).
    Let $\hat x_1, \hat x_2, \dots, \hat x_M$ be the sequence of experts that the adversary eliminates, that is, makes $\sum_{i=1}^t \ell(\hat x) \ge L\opt + 2 \alpha$.
    Note that the adversary is oblivious: that means that it can depend on the distribution of the exponential mechanism though it cannot depend on the returned expert $x_{t_1}$. In other words, $x_{t_1}$ is independent from $\hat x_1,\hat x_2,\dots,\hat x_M$. The goal is to upper bound $\P(M < N^{t_1}_j/2 \mid x_{t_1} \in S^{t_1}_j)$ or equivalently lower bound $\P(M \ge N^{t_1}_j/2 \mid x_{t_1} \in S^{t_1}_j)$. We have
    \begin{align*}
    &\P(M \ge N^{t_1}_j/2 \mid x_{t_1} \in S^{t_1}_j)
    \\
        & \ge \P( x_{t_1} \notin \{\hat x_1,\dots, x_{\floor{N^{t_1}_j/2}} \} \mid x_{t_1} \in S^{t_1}_j ) \\
        & = \P( x_{t_1} \in S^{t_1}_j \setminus \{\hat x_1,\dots,\hat x_{\floor{N^{t_1}_j/2}} \} \mid x_{t_1} \in S^{t_1}_j ) \\
        & \ge \frac{1}{2e} \ge \frac{1}{6}.
    \end{align*}
    The claim follows.
\end{proof}


We are now ready to prove~\cref{lemma:switching-shrinkage}.
\begin{proof}[of \cref{lemma:switching-shrinkage}]
    Let $p_j = \P(x_{t_1} \in S^{t_1}_j)$ be the probability that the exponential mechanism returns an expert in $S^{t_1}_j$. Noting that $\sum_{j=1}^B p_j = \P(x_{t_1} \in \Sg^{t_1}) \ge 1 - \beta \ge 1/2$, 
    %the probability of returning expert $x_{t_1} \in \Sb^{t_1}$ is at most $\beta \le 1/2$, 
    we have that there is $j \in [B]$ such that $ p_j \ge 1/2B$. On the other hand, $s_t(x) \le s_t(x')$ for $x \in S^{t_1}_j$ and $x' \in S^{t_1}_{j'} $, which implies that $\P(x_{t_1} = x) \ge \P(x_{t_1} = x')$. This implies that 
    \begin{equation*}
        \frac{1}{2 B} \le p_j \le \frac{N^{t_1}_j}{\sum_{\ell=1}^j N^{t_1}_\ell},
    \end{equation*}
    or stated differently 
    \begin{equation*}
        \frac{\sum_{\ell=1}^j N^{t_1}_\ell}{2 B} \le {N^{t_1}_j}.
    \end{equation*}
    If the exponential mechanism picks an expert $x_{t_1} \in S_j^{t_1}$ (which happens with probability $p_t \ge 1/2B$), \cref{lemma:adv-eliminiation} now implies that at the next switch at time $t_2$ with probability $1/6$ the adversary will eliminate $N^{t_1}_j/2$ experts from $S^{t_1}_j$ which implies
    \begin{align*}
    \sum_{\ell=1}^j N^{t_2}_\ell 
        %&  \le \sum_{\ell=1}^{i-1} N^{t'}_\ell + \frac{1}{4} N^{t'}_i\\
        & \le  \sum_{\ell=1}^{j} N^{t_1}_\ell -  \frac{1}{2} N^{t_1}_j  \\
        & \le \sum_{\ell=1}^{j} N^{t_1}_\ell -\frac{1}{4B} \sum_{\ell=1}^{j} N^{t_1}_\ell \\
        & = \sum_{\ell=1}^{j} N^{t_1}_\ell (1 - \frac{1}{4B}).
    \end{align*}
    This proves the claim.
\end{proof}
\end{comment}


\subsection{Adaptive algorithms for DP experts}
While~\cref{alg:SVT-zero-loss} achieves near-optimal loss for settings with low-loss experts, it requires the knowledge of the value of $L\opt$. As $L\opt$ is not always available in practice, our goal in this section is to develop an adaptive version of~\cref{alg:SVT-zero-loss} which obtains similar regret without requiring the knowledge of $L\opt$. Similarly to other online learning problems, we propose to use the doubling trick~\cite{KalaiVe05} to design our adaptive algorithms. We begin with an estimate $L\opt_1 = 1$ of $L\opt$. Then we apply~\cref{alg:SVT-zero-loss} using $L\opt = L\opt_1$ until the exponential mechanism picks an expert that contradicts the current estimate of $L\opt$, that is,  $\sum_{i=1}^{t-1} \ell_i(x_t) \gg L\opt_1$. We use the Laplace mechanism to check this privately. Noting that this happens with small probability if $L\opt \le L\opt_1$, we conclude that our estimate of $L\opt$ was too small and set a new estimate $L\opt_2 = 2 L\opt_1$ and repeat the same steps. As $L\opt \le T$, this process will stop in at most $\log T$ phases, hence we can divide the privacy budget equally among phases while losing at most a factor of $\log T$. We present the full details in~\Cref{alg:SVT-ada}.


\begin{algorithm}[t]
	\caption{Adaptive Sparse-Vector for low-loss experts }
	\label{alg:SVT-ada}
	\begin{algorithmic}[1]
		\REQUIRE Failure probability $\beta$
            \STATE Set $\diffp_0 = \diffp / 2\log T$, $\beta_0 = \beta/T$
		\STATE $K = 6\ceil{\log d} +  24 \log(1/\beta_0)$, $\eta = \diffp_0/2K$, $B =  \log(2T^2/\beta_0)$	
            \STATE Set $\bar L\opt = 1$, $L = L\opt + 4/\eta + \frac{8B}{\diffp_0}$
        \WHILE{$t < T$}
            \STATE Run~\Cref{alg:SVT-zero-loss} with parameters $\bar  L\opt$, $\eta$,  $L$, $\beta_0$, $\diffp_0$ 
            \IF{\Cref{alg:SVT-zero-loss} applies the exponential mechanism (step 12)}
                \STATE Calculate $\bar L_t = \sum_{i=1}^{t-1} \ell_i(x_t) + \zeta_t$ where $\zeta_t \sim \lap(K/\diffp_0)$
                \IF{$\bar L_t  > \bar  L\opt - 5K\log(1/\beta_0)/\diffp_0 $}
                    \STATE Set $\bar  L\opt = 2 \bar 
 L\opt$
                    \STATE Go to step 4
                \ENDIF
            \ENDIF
        \ENDWHILE
	\end{algorithmic}
\end{algorithm}

We have the following guarantees for the adaptive algorithm.
\iftoggle{arxiv}{}{
We defer the proof to~\Cref{sec:proof-ub-realizable-ada}.
}
\begin{theorem}
\label{thm:ub-realizable-ada}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary such that there is $x\opt \in [d]$ such that $\sum_{t=1}^T \ell_t(x\opt) \le L\opt$. Let $0 < \beta < 1/2$. Then
    \Cref{alg:SVT-ada} is $\diffp$-DP and with probability at least $1-O(\beta)$ has regret 
    \iftoggle{arxiv}{
    \begin{equation*}
        \sum_{t=1}^T \ell_t(x_t) \le O\left(  L\opt \log(Td/\beta) \log(T) + \frac{\log^2(d)\log(T) + \log(T/\beta) \log(Td/\beta) \log(T)}{\diffp}  \right).
    \end{equation*}
    }
    {
    \begin{align*}
    & \sum_{t=1}^T \ell_t(x_t) \le O\left(  L\opt \log(Td/\beta) \log(T) \right) \\ 
    & + O\left( \frac{\log^2(d)\log(T) + \log(T/\beta) \log(Td/\beta) \log(T)}{\diffp}  \right).
    \end{align*}
    }
\end{theorem}
\iftoggle{arxiv}{
\begin{proof}
    First we prove privacy. Note that $\bar L\opt$ can change at most $\log(T)$ times as $L\opt \le T$. Therefore, we have at most $\log(T)$ applications of~\Cref{alg:SVT-zero-loss}. Each one of these is $\diffp/(2\log(T))$-DP. Moreover, since we have at most $K$ applications of the exponential mechanism in~\Cref{alg:SVT-zero-loss}, we have at most $K \log(T)$ applications of the Laplace mechanism in~\Cref{alg:SVT-ada}. Each of these is $\diffp/2K\log(T)$-DP. Overall, privacy composition implies that the final privacy is $\diffp$-DP.

    Now we prove utility. \Cref{alg:SVT-ada} consists of at most $\log(T)$ applications of~\Cref{alg:SVT-zero-loss} with different values of $\bar L\opt$. We will show that each of these applications incurrs low regret.
    Consider an application of~\Cref{alg:SVT-zero-loss} with $\bar L\opt$. If $\bar L\opt \ge L\opt$, then~\Cref{thm:ub-realizable} implies that the regret is at most $$O\left( \bar L\opt \log(d/\beta_0) + \frac{\log^2(d) + \log(T/\beta_0) \log(d/\beta_0)}{\diffp_0}  \right).$$ 
    Now consider the case where $\bar L\opt \le L\opt$. We will show that~\Cref{alg:SVT-ada} will double $\bar L\opt$ and that the regret of~\Cref{alg:SVT-zero-loss} up to that time-step is not too large.
    Let $t_0$ be the largest $t$ such that $\min_{x \in [d]} \sum_{t=1}^{t_0} \ell_t(x) \le \bar L\opt$. Note that up to time $t_0$, the best expert had loss at most $\bar L\opt$ hence the regret up to time $t_0$ is $$O\left( \bar L\opt \log(d/\beta_0) + \frac{\log^2(d) + \log(T/\beta_0) \log(d/\beta_0)}{\diffp_0}  \right).$$ 
    Now let $t_1$ denote the next time-step when~\Cref{alg:SVT-zero-loss} applies the exponential mechanism. Sparse-vector guarantees that in the range $[t_0,t_1]$ the algorithm suffers regret at most $O\left( \bar L\opt  + \frac{\log(d) + \log(T/\beta_0) }{\diffp_0}  \right)$. Moreover, the guarantees of the Laplace mechanism imply that at this time-step, $\bar L_t \ge \bar  L\opt - 5K\log(1/\beta_0)/\diffp_0$ with probability $1-\beta_0$, hence~\Cref{alg:SVT-ada} will double $\bar L\opt$ and run a new application of~\Cref{alg:SVT-zero-loss}. Overall, an application of~\Cref{alg:SVT-zero-loss} with $\bar L\opt \le L\opt$ results in regret $(L\opt + \frac{1}{\diffp_0}) \cdot \mathsf{poly} (\log \frac{Td}{\beta_0})$ and doubles $\bar L\opt$. Finally, note that if $\bar L\opt \ge L\opt + 5\log(1/\beta_0)/\diffp_0$ then with probability $1-\beta_0$ the algorithm will not double the value of $\bar L\opt$. As each application of ~\Cref{alg:SVT-zero-loss} has regret $$O\left( \bar L\opt \log(d/\beta_0) + \frac{\log^2(d) + \log(T/\beta_0) \log(d/\beta_0)}{\diffp_0}  \right),$$ and $\bar L\opt$ is bounded by $L\opt + 5\log(T/\beta_0)/\diffp_0$ with probability $1 - O(\beta_0)$. Overall, the failure probability is $O(T \beta_0) = O(\beta)$. \ha{go over this proof again..}
\end{proof}
}

\iftoggle{arxiv}{}{We also present a different binary-tree based mechanism for this problem with similar rates in~\Cref{sec:bt-experts}.}

\iftoggle{arxiv}{
\subsection{A binary-tree based algorithm}

In this section, we present another algorithm which achieves the optimal regret for settings with zero-expert loss. Instead of using sparse-vector, this algorithm builds on the binary tree mechanism. The idea is to repetitively select $O(\mathsf{poly}(\log(dT)))$ random good experts and apply the binary tree to calculate a private version of their aggregate losses. Whenever all of the chosen experts are detected to have non-zero loss, we choose a new set of good experts. Similarly to~\cref{alg:SVT-zero-loss}, we can show that each new phase reduces the number of good experts by a constant factor as an oblivious adversary does not know the choices of the algorithm, hence there are only $O(\mathsf{poly}(\log(dT)))$ phases. 


We provide a somewhat informal description of the algorithm in~\cref{alg:Bin-tree-zero-loss}. This algorithm also achieves regret $O(\mathsf{poly}(\log(dT))/\diffp)$ in the realizable case. We do not provide a proof as it is somewhat similar to that of~\cref{thm:ub-realizable}.
\begin{algorithm}
	\caption{Binary-tree algorithm for zero loss experts (sketch)}
	\label{alg:Bin-tree-zero-loss}
	\begin{algorithmic}[1]
		%\REQUIRE Data points $\Ds=(\ds_1, \ldots, \ds_n)\in \domain^n$,
		%constraint set $\xdomain$,
		%step size $\ss$, initial point $x_0$;
		\STATE Set $k=0$ and $B=  O(\mathsf{poly}(\log(dT)))$
        \WHILE{$t \le T$\,}
            \STATE Use the exponential mechanism with score function $s(x) = \sum_{i=1}^t \ell_i(x)$ to privately select a set $S_k$ of $B$ experts from $[d] \setminus \cup_{0 \le i \le k} S_i$
            \STATE Apply binary tree for each expert $x \in S_k$ to get private aggregate estimates for $ \sum_{i=1}^t \ell_i(x)$ for every $t \in [T]$
            \STATE Let $\hat c_{t,x}$ denote the output of the binary tree for expert $x \in S_k$ at time $t$ 
            \WHILE{there exists $x \in S_k$ such that $\hat c_{t,x} \le O(\mathsf{poly}(\log(dT))/\diffp)$}
                \STATE Receive $\ell_t : [d] \to [0,1]$
                \STATE Choose $x_t \in S_k$ that minimizes $\hat c_{t,x}$
        	    \STATE Pay error $\ell_t(x_t)$
        	    \STATE $t = t+1$
            \ENDWHILE
            \STATE $k = k + 1$
        \ENDWHILE
	\end{algorithmic}
\end{algorithm}
}

%We provide the proof in the appendix as it is similar to the proof of~\cref{thm:ub-realizable}.
% \begin{theorem}
% \label{thm:ub-realizable-alt}
%     Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary such that there is $x\opt \in [d]$ such that $\sum_{t=1}^T \ell_t(x\opt) = 0$. Then
%     \cref{alg:Bin-tree-zero-loss} is \ed-DP and has regret 
%     \begin{equation*}
%         \sum_{t=1}^T \ell_t(x_t) \le O\left( \frac{\mathsf{poly} (\log d)}{\diffp} \right).
%     \end{equation*}
% \end{theorem}


% \begin{comment}

% \subsection{Adaptive algorithms for $L\opt > 0$}
% Motivated by the improvements for the realizable setting, in this section we develop algorithms that are adaptive to the loss of the best expert. More precisely, if the best expert has loss $L\opt = \min_{x \in [d]} \sum_{t=1}^T \ell_t(x)$ then our algorithms achieve regret $O\left(L\opt \log(T) + \frac{\mathsf{poly} (\log d)}{\diffp} \right)$.

% Our algorithm in this section builds on the algorithm for the realizable case using the doubling trick: we start with a small estimate $L\opt_0 = 1$ of the loss of the best expert and double this loss whenever the algorithm identifies that all experts has loss worse than $L\opt_0$. \cref{alg:adaptive-loss} describes the full details of this algorithm.



% \begin{algorithm}
% 	\caption{Adaptive sparse-vector algorithm}
% 	\label{alg:adaptive-loss}
% 	\begin{algorithmic}[1]
% 		%\REQUIRE Data points $\Ds=(\ds_1, \ldots, \ds_n)\in \domain^n$,
% 		%constraint set $\xdomain$,
% 		%step size $\ss$, initial point $x_0$;
% 		\STATE Set current expert $x_0 = \mathsf{Unif}[d]$	
% 		\STATE Set $k=0$, $L\opt_0 = 1$, and $count=0$
%         \FOR{$t=1$ to $T$\,}
%             \STATE Set $ x_{t} =  x_{t-1}$
%                 \STATE Run a Sparse-Vector query to identify if $\sum_{i=1}^{t-1} \ell_i(x_t) \ge L\opt_k + \frac{100 \log(d)}{\diffp}$
%                 \IF{Sparse-Vector identifies above threshold}
%                     \STATE $count = count + 1$
%                     \STATE Run exponential mechanism with scores $s(x) = \sum_{i=1}^{t-1} \ell_i(x)$ for $x \in [d]$ 
%                     \STATE Let $ x_{t}$ be the output of the exponential algorithm
%                     % \STATE Calculate $\hat s_t = \sum_{i=1}^{t-1} \ell_i(x_t) + \mathsf{Laplace}(\log(T)/\diffp)$
%                     % \IF{$\hat s_t \ge 2 L\opt_k + \frac{100 \log(d)}{\diffp}$}
%                     %     \STATE $L\opt_{k+1} = 2L\opt_k$
%                     %     \STATE $k = k+1$
%                     % \ENDIF
%                 \ENDIF
%             \IF{$count \ge 100 \log^4(d)$}
%                 \STATE $L\opt_{k+1} = 2 L\opt_k$
%                 \STATE $k = k+1$
%                 \STATE $count = 0$
%             \ENDIF
%         	\STATE Receive loss function $\ell_t: [d] \to [0,1]$
%         	\STATE Pay cost $\ell_t(x_t)$
%         \ENDFOR
% 	\end{algorithmic}
% \end{algorithm}


% The following theorem states our adaptive upper bound for~\cref{alg:adaptive-loss}. We provide the proof in~\cref{sec:proof-thm-ub-adaptive}.
% \begin{theorem}
% \label{thm:ub-adaptive}
%     Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary and denote $L\opt = \min_{x \in [d] }\sum_{t=1}^T \ell_t(x)$. Then
%     \cref{alg:adaptive-loss} is \ed-DP and has regret 
%     \begin{equation*}
%         \sum_{t=1}^T \ell_t(x_t) \le O\left(L\opt \log(T) + \frac{\mathsf{poly} (\log d)}{\diffp} \right).
%     \end{equation*}
%     \hac{prove this. first term might need $\log d$ factors?}
% \end{theorem}

% % \begin{remark}
% %     We can generalize this algorithm for $L\opt = \min_{j \in [d]} \sum_{t=1}^n z_{t,j} >0$ to get regret roughly
% %     \begin{equation*}
% %         \mathsf{Regret} \le O\left(L\opt \log d + \frac{\mathsf{poly} (\log d)}{\diffp} \right).
% %     \end{equation*}
% %     The idea is to apply the previous algorithm for $L\opt_0 = 0$ until all experts are bad. Then we increase $L\opt_{k+1} = 2L\opt_k + 1 $ and repeat the previous algorithm. This will achieve the desired regret.
% % \end{remark}
% 
% \end{comment}

